Improved Exploration in Factored Average-Reward MDPs

We consider a regret minimization task under the average-reward criterion in an unknown Factored Markov Decision Process (FMDP). More specifically, we consider an FMDP where the state-action space $\mathcal X$ and the state-space $\mathcal S$ admit the respective factored forms of $\mathcal X = \otimes_{i=1}^n \mathcal X_i$ and $\mathcal S=\otimes_{i=1}^m \mathcal S_i$, and the transition and reward functions are factored over $\mathcal X$ and $\mathcal S$. Assuming known factorization structure, we introduce a novel regret minimization strategy inspired by the popular UCRL2 strategy, called DBN-UCRL, which relies on Bernstein-type confidence sets defined for individual elements of the transition function. We show that for a generic factorization structure, DBN-UCRL achieves a regret bound, whose leading term strictly improves over existing regret bounds in terms of the dependencies on the size of $\mathcal S_i$'s and the involved diameter-related terms. We further show that when the factorization structure corresponds to the Cartesian product of some base MDPs, the regret of DBN-UCRL is upper bounded by the sum of regret of the base MDPs. We demonstrate, through numerical experiments on standard environments, that DBN-UCRL enjoys substantially improved regret empirically over existing algorithms that have frequentist regret guarantees.

==> sections/algo_arXiv.tex <==

\section{The \AlgB\ Algorithm}\label{sec:algo}

%\vspace{-2mm}\noindent
%In this section we present the \AlgB\ algorithm. %Since \AlgB\ is a model-based algorithm that implements the optimistic principle as in other similar algorithms such as UCRL2 \citep{jaksch2010near}, 

%\vspace{-2mm}\noindent
\subsection{Confidence Sets for Factored MDPs}
%\vspace{-2mm}\noindent
We begin with introducing empirical estimates and confidence sets used by \AlgB. Throughout this section, for each given $Z\!\subseteq\! [n]$ and $x\!\in\! \cX[Z]$, we let  $\text{N}(t, x; Z) := \max(\sum_{t'=1}^{t-1} \indic{x_{t'}[Z] = x}, 1)$ denote the number of visits to $x$ up to time $t$.


%\vspace{-2mm}\noindent
\paragraph{Empirical Estimates for Factored Representation} 
%State at time $t$ is $s_t$. Action at time $t$ is $a_t$. 
Let us consider time $t\ge 1$ and recall that $x_t = (s_t, a_t)$. 
For $i\!\in\! [m]$ we define the shorthand notation $N^p_{i,t}(x):= \text{N}(t, x; Z^p_i)$. Likewise, for $i\!\in\! [\ell]$ we define $N^r_{i,t}(x):= \text{N}(t, x; Z^r_i)$.
We then introduce the following empirical estimates:
Given $i\!\in\! [m], x\!\in\! \cX[Z^p_i]$, we let $\widehat P_{i,t}(\cdot|x)$  be the empirical distribution built using $N^p_{i,t}(x)$ i.i.d.~samples from $P_{i}(\cdot|x)$:
%\vspace{-3mm}\noindent
%for all $i\in [m]$, for all $x\in \cX[Z^p_i],$ and for all $y\in \cS_i$,
\begin{align*}
\widehat P_{i,t}(y|x) &:= \frac{1}{N^p_{i,t}(x)} \sum_{t'=1}^{t-1} \indic{x_{t'}[Z^p_i] = x, s_{t'+1}[i] = y}\, .
\end{align*}
Similarly, 
given $i\in [\ell]$ and $x\in \cX[Z^r_i]$, we define $\widehat \mu_{i,t}(x)$ as the empirical estimate of $R_i(x)$ built using $N^r_{i,t}(x)$ i.i.d.~samples from $R_i(x)$: 
%and for all $i\in [\ell]$ and $x\in \cX[Z^r_i]$, 
%& \quad \forall i\in [m],\, \forall x\in \cX[Z^p_i],\, \forall y\in \cS_i, \\
\begin{align*}
\widehat\mu_{i,t}(x) &:= \frac{1}{N^r_{i,t}(x)} \sum_{t'=1}^{t-1} r_{t'}[i]\indic{x_{t'}[Z^r_i] = x}\, .
%&\quad\quad\quad \forall i\in [\ell],\, \forall x\in \cX[Z^r_i].
\end{align*}

%\vspace{-3mm}\noindent
\paragraph{Local Confidence Sets}
We first define the confidence set for the reward function. For each $i\in [\ell]$ and $x\in \cX[Z_i^r]$, we introduce the following entry-wise confidence sets
\als{
&c_{t,\delta,i}(x) =\bigg\{q\in[0,1]:|\widehat \mu_{i,t}(x)  - q| \le
\sqrt{\frac{2\widehat\sigma_{i,t}^2(x)}{N^r_{i,t}(x)}\beta_{N^r_{i,t}(x)}(\delta)} \!+\! \frac{7\beta_{N^r_{i,t}(x)}(\delta)}{3N^r_{i,t}(x)}
 \bigg\}\,,
}
%where we introduce the notation
%\als{
%\beta^r_{t,i}(\delta):= &\max\bigg\{\tfrac{1}{2} \beta'_{N^r_{i,t}(x)}(\delta), \sqrt{\frac{2\widehat\sigma_{i,t}^2(x)}{N^r_{i,t}(x)}\beta_{N^r_{i,t}(x)}(\delta)} \!+\! \frac{7\beta_{N^r_{i,t}(x)}(\delta)}{3N^r_{i,t}(x)}\bigg\}\,.
%}
where $\widehat\sigma^2_{i,t}(x)$ denotes the empirical variance of the reward function $R_i(x)$ built using the observations gathered up to time $t$, and for $n\in \NN$ and $\delta\in (0,1)$, we define 
\als{
\beta_n(\delta) &:= \eta\log\Big(\frac{\log(n)\log(\eta n)}{\log^2(\eta)\delta}\Big)\, , %\hbox{ }  %\quad 
%\beta'_n(\delta)&:=\sqrt{ \frac{2(1+\frac{1}{n})\log(\sqrt{n+1}/\delta)}{n}}\, .
}
with $ \eta\!=\!1.12$. The definition of the confidence set $c_{t,\delta,i}(x)$ is obtained a Bernstein concentration inequality, modified using a peeling technique to handle arbitrary random stopping times.\footnote{We refer the interested reader to \citep{maillard2019mathematics} for the generic proof technique behind this result. It is also worth noting that \citep{dann2017unifying} uses a similar proof technique for Bernstein concentrations, but with looser bounds.} We also note that in the definition of $\beta_n(\delta)$, any choice of $\eta>1$ is valid, however $\eta=1.12$ yields a small bound.\footnote{The optimal $\eta$ is obtained by optimizing $\beta_n(\delta)$ over $\eta$. The optimal $\eta$ will depend on $n$, but as $\beta_n(\delta)$ grows very slowly with $n$, the optimal $\eta$ can be approximated well by a constant function $\eta=1.12$.} 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
% See the commented lines below for the version with joint Laplace-Bernstein CIs
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%We first define the confidence set for the reward function. For each $i\in [\ell]$ and $x\in \cX[Z_i^r]$, we introduce the following entry-wise confidence sets
%\als{
%%\label{eq:L1_CB}
%c_{t,\delta,i}(x) =\Big\{q\in[0,1]:|\widehat \mu_{i,t}(x)  - q| \le \beta^r_{t,i}\big(\tfrac{\delta}{3\ell|\cX[Z^r_i]|}\big)\Big\}\,,
%}
%where we introduce the notation
%\als{
%\beta^r_{t,i}(\delta):= &\max\bigg\{\tfrac{1}{2} \beta'_{N^r_{i,t}(x)}(\delta), \sqrt{\frac{2\widehat\sigma_{i,t}^2(x)}{N^r_{i,t}(x)}\beta_{N^r_{i,t}(x)}(\delta)} \!+\! \frac{7\beta_{N^r_{i,t}(x)}(\delta)}{3N^r_{i,t}(x)}\bigg\}\,.
%}
%Here $\widehat\sigma^2_{i,t}(x)$ denotes the empirical variance of the reward function $R_i(x)$ built using the observations gathered up to time $t$, and for $n\in \NN$ and $\delta\in (0,1)$, we define 
%\als{
%\beta_n(\delta) &:= \eta\log\Big(\frac{\log(n)\log(\eta n)}{\log^2(\eta)\delta}\Big) \hbox{ with $ \eta\!=\!1.12$, and}  \\ %\quad 
%\beta'_n(\delta)&:=\sqrt{ \frac{2(1+\frac{1}{n})\log(\sqrt{n+1}/\delta)}{n}}\, .
%}
%The definition of the confidence set $c_{t,\delta,i}(x)$ is obtained by combining (i) a Hoeffding-type concentration inequality for random variables in $[0,1]$, modified to hold for an arbitrary random stopping time, using the method of mixture (a.k.a.~the Laplace method) from \cite{pena2008self}; and (ii) a Bernstein concentration inequality, modified using a peeling technique in order to handle arbitrary random stopping times.\footnote{We refer the interested reader to \cite{maillard2019mathematics} for the generic proof technique behind this result. It is also worth noting that \cite{dann2017unifying} uses a similar proof techniques for Bernstein concentrations, but with looser bounds.} We also note that in the definition of $\beta_n(\delta)$, any choice of $\eta>1$ is valid, however $\eta=1.12$ yields a small bound.\footnote{{\color{blue}The best $\eta$ is obtained by optimizing $\beta_n(\eta)$ over $\eta$. The optimal $\eta$ will depend on $n$, but as $\beta_n(\delta)$ grows very slowly with $n$, the optimal $\eta$ turns out to be a near-constant function of $n$ (in other words, it can be approximated well by a constant function)
%, and $\eta=1.12$ is a good approximation of this near-constant function.}} 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%The definition of the confidence set $c_{t,\delta,i}(x)$ is obtained by combining (i) is motivated by Hoeffding-type concentration inequalities for $1/2$-sub-Gaussian distributions\footnote{Random variables bounded in $[0,1]$ are $\tfrac{1}{2}$-sub-Gaussian.}, modified to hold for an arbitrary random stopping time, using the method of mixture (a.k.a.~the Laplace method) from \cite{pena2008self}. It is further combined with a Bernstein concentration inequality, modified using a peeling technique in order to handle arbitrary random stopping times. We refer the interested reader to \cite{MaillardHDR} for the generic proof technique behind this result\footnote{In  \cite{dann2017unifying}, the authors used similar proof techniques for Bernstein concentrations, but with looser bounds.}. 
%Any choice of $\eta>1$ is valid, however $\eta=1.12$ yields a small bound. The definition of the confidence set $c_{t,\delta,i}(x)$ is motivated by Hoeffding-type concentration inequalities for $1/2$-sub-Gaussian distributions\footnote{Random variables bounded in $[0,1]$ are $\tfrac{1}{2}$-sub-Gaussian.}, modified to hold for an arbitrary random stopping time, using the method of mixture (a.k.a.~the Laplace method) from \cite{pena2008self}. It is further combined with a Bernstein concentration inequality, modified using a peeling technique in order to handle arbitrary random stopping times. We refer the interested reader to \cite{MaillardHDR} for the generic proof technique behind this result\footnote{In  \cite{dann2017unifying}, the authors used similar proof techniques for Bernstein concentrations, but with looser bounds.}. 
%
% This satisfies by construction that
This leads us to define the following confidence set for mean rewards: For $x\in \cX$,
%\vspace{-2mm}\noindent
\als{
&\cC^r_{t,\delta}(x)\!=\!\bigg\{\!\mu'\in \cR_{\cX,[0,1]}^{\textrm{fac}}(\cG_r): \forall i\in [\ell], \mu'_i(x[Z^r_i]) \in c_{t,\delta_i,i}(x[Z^r_i]) \! \bigg\}.
}
where $\delta_i = \delta(2\ell |\cX[Z^r_i]|)^{-1}$. 
%\vspace{-2mm}\noindent
As for the transition function, we define for each $i\!\in\! [m]$, $x\!\in\! \cX[Z^p_i]$ and $y\!\in\! \cS_i$ the confidence set:
%\vspace{-2mm}\noindent
\als{
C_{t,\delta,i}(x,y)\!=\! \bigg\{\! q\!\in\![0,1]\!:  | \widehat P_{i,t}(y|x) - q | 
 \!\le\! \sqrt{\frac{2q(1\!-\!q)}{N^p_{i,t}(x)}\beta_{N^p_{i,t}(x)}(\delta_i)} \!+\! \frac{\beta_{N^p_{i,t}(x)}(\delta_i)}{3N^p_{i,t}(x)}
\bigg\}\,, 
%&C^2_{t,\delta,i}(x,y)\!=\! \bigg\{\! q\!\in\![0,1]\!:  -\sqrt{\underline{g}(q)}\beta'_{N^p_{i,t}(x)}(\delta_i) \!\le \widehat P_{i,t}(y|x) - q \!\le\! \sqrt{g(q)} \beta'_{N^p_{i,t}(x)}(\delta_i)
%\bigg\}\,,
}
%\als{
%&C^1_{t,\delta_0,i}(x,y)\!=\! \bigg\{\! q\!\in\![0,1]\!:  | \widehat P_{i,t}(y|x) - q |
% \!\le\! \sqrt{\frac{2q(1\!-\!q)}{N_t(x)}\beta_{N_t(x)}\big(\tfrac{\delta_0}{S_i|\cX[Z_i]|}\big)} \!+\! \frac{\beta_{N_t(x)}\big(\tfrac{\delta_0}{S_i|\cX[Z_i]|}\big)}{3N_t(x)}
%\bigg\}\,, \\
%&C^2_{t,\delta_0,i}(x,y)\!=\! \bigg\{\! q\!\in\![0,1]\!:  -\sqrt{\underline{g}(q)}\beta_{N_t(x)}\big(\tfrac{\delta_0}{S_i|\cX[Z_i]|}\big) \!\le \widehat P_{i,t}(y|x) - q \!\le\! \sqrt{g(q)} \beta_{N_t(x)}\big(\tfrac{\delta_0}{S_i|\cX[Z_i]|}\big)
%\bigg\}\,,
%}
where $\delta_i = \delta(2mS_i|\cX[Z^p_i]|)^{-1}$. %, and where $\underline{g}(p)\!=\!\begin{cases} g(p)&\text{if }p\!<\!0.5\\ p(1\!-\!p) &\text{else}\end{cases}\!,$ with $g(p) \!=\! \frac{1/2-p}{\log(1/p\!-\!1)}$. 
This construction  comes from a Bernstein concentration inequality as above.  %and the set $C^2$ is derived by applying again the method of mixture (a.k.a.~the Laplace method) for sub-Gaussian random variables, with a modification: Indeed Bernlli random variables are not only $1/2$-sub-Gaussian, but satisfy a stronger sub-Gaussian tail property, already observed in \cite{berend2013concentration,raginsky2013concentration}. 
%The set $C^1$  comes from a Bernstein concentration inequality as above, and the set $C^2$ is derived by applying again the method of mixture (a.k.a.~the Laplace method) for sub-Gaussian random variables, with a modification: Indeed Bernlli random variables are not only $1/2$-sub-Gaussian, but satisfy a stronger sub-Gaussian tail property, already observed in \cite{berend2013concentration,raginsky2013concentration}.  
%where for $n\in \NN$ and $\delta\in (0,1)$, we define $\beta_n(\delta) \!=\! \eta\log\Big(\frac{\log(n)\log(\eta n)}{\log^2(\eta)\delta}\Big)$ with $\eta\!=\!1.12$.\footnote{Any $\eta>1$ is valid, and $\eta=1.12$ yields a small bound.} 
Finally, we define the confidence set for $P$ as follows: For $x\in \cX$,
%\vspace{-2mm}\noindent 
\als{
\cC^p_{t,\delta}(x)\!=\!\bigg\{&\!P'\in \cP_{\cX,\cS}^{\textrm{fac}}(\cG_p): \forall i\in [m], \forall y\in \cS_i,  P'_i(y|x[Z^p_i]) \in C_{t,\delta,i}(x[Z^p_i],y) \! \bigg\}\, .
}
%\als{
%\cC_{t,\delta}(x)\!=\!\bigg\{\!P'\in \cP_{\cX,\cS}^{\textrm{fac}}(\cG_p): \forall i\in [m], \forall y\in \cS_i,  P'_i(y|x[Z^p_i]) \in C^1_{t,\delta,i}(x[Z^p_i],y) \cap C^2_{t,\delta,i}(x[Z^p_i],y) \! \bigg\}\, .
%}

%\vspace{-2mm}\noindent
By construction, these confidence sets contain the reward and transition functions of the true FMDP $M$ with probability at least $1-2\delta$, and in particular, this holds uniformly for all time horizons $T$. (We present a formal statement of this fact in Appendix~\ref{app:concentration_inequalities} in the supplementary material.) 

%Let us choose $\delta_0 = \delta/(3+3S)$. \footnote{When an upper bound $\overline{K}$ over $\max_{s,a} K_{s,a}$ is known, one could choose the confidence level $\delta_0 = \delta/(3+3\overline{K})$.} 
%The following lemma states that with high probability, the reward and transition functions of the true MDP $M$ are contained in $\cM_{t,\delta}$ for all $t\in \NN$:
%
%\begin{lemma}[Time-uniform confidence bounds]\label{lem:CI_has_trueMDP}
%	For any FMDP with rewards in $\cR^{\text{fac}}_{\cX,[0,\ell]}(\cG_r)$, and transition function in $\cP^{\text{fac}}_{\cX,\cS}(\cG_p)$, for all $\delta\in(0,1)$, it holds
%\als{
%&\Pr\bigg(\exists t\in\Nat, x\in \cX, \quad  \mu(x) \notin c_{t,\delta}(x)
%	\,\,\text{ or } \,\,P(\cdot|x) \notin \cC_{t,\delta}(x)\bigg)\leq 2\delta\,.
%}
%%For all $\delta\in (0,1)$, it holds that
%%$$
%%\PP\big(\exists t\in \NN, M\notin \cM_{t,\delta}\big)\leq 2\delta.
%%$$ 
%\end{lemma}

%\vspace{-2mm}\noindent
\subsection{\AlgB: Pseudo-code}
%\vspace{-2mm}\noindent
\AlgB\ receives the structure $\cG(M)$ of the true FMDP $M$ as input. In order to implement the optimistic principle, \AlgB\ considers the following set of plausible FMDPs at time $t$:
\als{
\cM_{t,\delta}=\Big\{M'=(\cS,\cA,P',R') \in \mathbb M_{\cG(M)}:  \mu'(x) \in \cC^r_{t,\delta}(x) \hbox{ and } P'(\cdot|x) \in\cC^p_{t,\delta}(x), \, \forall x\in \cX\Big\}\, .
} 
By construction of the confidence sets, the set $\cM_{t,\delta}$ contains the true FMDP with high probability: Formally, $\PP\big(\exists t\!\in\! \NN, M\!\notin\! \cM_{t,\delta}\big)\leq 2\delta$.
%Let us choose $\delta_0 = \delta/(3+3S)$. \footnote{When an upper bound $\overline{K}$ over $\max_{s,a} K_{s,a}$ is known, one could choose the confidence level $\delta_0 = \delta/(3+3\overline{K})$.} 
%The following lemma states that with high probability, the reward and transition functions of the true MDP $M$ are contained in $\cM_{t,\delta}$ for all $t\in \NN$:
%
%\begin{lemma}[Time-uniform confidence bounds]\label{lem:CI_has_trueMDP}
%	For any FMDP with rewards in $\cR^{\text{fac}}_{\cX,[0,\ell]}(\cG_r)$, and transition function in $\cP^{\text{fac}}_{\cX,\cS}(\cG_p)$, for all $\delta\in(0,1)$, it holds
%\als{
%&\Pr\bigg(\exists t\in\Nat, x\in \cX, \quad  \mu(x) \notin c_{t,\delta}(x)
%	\,\,\text{ or } \,\,P(\cdot|x) \notin \cC_{t,\delta}(x)\bigg)\leq 2\delta\,.
%}
%%For all $\delta\in (0,1)$, it holds that
%%$$
%%\PP\big(\exists t\in \NN, M\notin \cM_{t,\delta}\big)\leq 2\delta.
%%$$ 
%\end{lemma}
The algorithm aims to compute the optimal policy $\overline\pi^+_t$ among all policies in all plausible FMDPs in $\cM_{t,\delta}$, that is $\overline{\pi}_t^+ \!=\! \argmax_{\pi:\cS\to\cA} \max\{ g_\pi^M\!:  M \!\in\! \cM_{t,\delta} \}$, where $g_\pi^M$ is the gain for policy $\pi$ in FMDP $M$. This is carried out approximately by Extended Value Iteration (\EVI) that builds a near-optimal policy $\pi^+_t$ and an FMDP $\widetilde M_t$ such that $g_{\pi^+_t}^{\widetilde M_t}  \geq \max_{\pi,  M\in\cM_{t,\delta} }g_\pi^M - \tfrac{1}{\sqrt{t}}$. Similarly to UCRL2 and its variants, \AlgB\ proceeds in internal episodes $k=1,2,\ldots$, where a near-optimistic policy $\pi_t^+$ is computed only at the starting time of each episode. Letting $t_k$ denote the starting time of episode $k$, the algorithm computes $\pi_k^+:=\pi_{t_k}^+$ and applies it until $t=t_{k+1}-1$, where $t_{k+1}$ is the first time step where the number of observations gathered on some reward factor or transition factor within episode $k$ is doubled. This event writes a bit differently in the FMDP setup. Namely, the sequence $(t_k)_{k\geq 1}$ is defined as follows: $t_1=1$, and for each $k>1$
\als{
t_k  &= \min\bigg\{ t > t_{k-1}:  \max\Big\{\max_{x\in \cX[Z^p_i], i\in [m]} \frac{\nu^p_{i, t_{k-1}:t}(x)}{N^p_{i,t_{k-1}}(x)}, \max_{x\in \cX[Z^r_i], i\in [\ell]} \frac{\nu^r_{i, t_{k-1}:t}(x)}{N^r_{i,t_{k-1}}(x)}\Big\}\geq 1 \bigg\},
}
where $\nu^p_{i, t_1:t_2}(x)$ (resp.~$\nu^r_{i, t_1:t_2}(x)$) denotes the number of observations of $x\!\in\! \cX[Z^p_i]$ (resp.~of $x\!\in\! \cX[Z^r_i]$) between time $t_1$ and $t_2$.%, and where we recall that for $x\!\in\! \NN$, $x^+\!:=\! \max\{x,1\}$.
The pseudo-code of \AlgB\ is provided in Algorithm \ref{alg:FMDP_UCRL2B}, and \EVI\ is presented in Algorithm \ref{alg:EVI}. % the supplementary.
In each round $n$, \EVI\ requires computing a factored transition function $\widetilde P_{n}$ such that for all $x=(s,a)$, $\widetilde P_n(\cdot|x) \in \argmax \{ \sum_{y\in \cS} P'(y)u_n(y):  P'\!\in\! \cC(x)\}$. This is carried out using \texttt{InnerMax}, whose pseudo-code is provided in Algorithm \ref{alg:InMax}. 


\begin{algorithm}[!hbtp]
   \caption{\AlgB}
   \label{alg:FMDP_UCRL2B}
   \small
\begin{algorithmic}
\STATE \textbf{Input:} Structure $\cG$, confidence parameter $\delta$
   \STATE \textbf{Initialize:} For all $i\in [m], x\in \cX[Z^p_i]$, set $N^p_{i,0}(x)=0$. For all $i\in [\ell], x\in \cX[Z^r_i]$, set $N^r_{i,0}(x)=0$. Set $t_0=0$, $t=1$, $k=1$.
   \FOR{episodes $k=1,2,\ldots$}
       \STATE Set $t_k = t$
      % \STATE For all $i\in [m], x\in \cX[Z^p_i]$, set $N^p_{i,t_k}(x) = N^p_{i,t_{k-1}}(x)+ \nu^p_{i,k-1}(x)$
      % \STATE For all $i\in [\ell], x\in \cX[Z^r_i]$, set $N^r_{i,t_k}(x) = N^r_{t_{k-1}}(x)+ \nu^r_{i,k-1}(x)$
       \STATE Compute empirical estimates $\{\widehat \mu_{i,t_k}(x)\}_{i\in [\ell], x\in\cX[Z^r_i]}$ and $\{\widehat P_{i,t_k}(\cdot|x)\}_{i\in [m], x\in \cX[Z_i^p]}$
       \STATE Compute $\pi^+_{k} = \EVI\Big(\cC^r_{t_k,\delta}, \cC^p_{t_k,\delta}, \tfrac{1}{\sqrt{t_k}}\Big)$ -- see Algorithm \ref{alg:EVI} %in the supplementary.
       \STATE Set $\nu^p_{i,k}(x)=0$ for all $i\in[m]$ and $x\in \cX[Z_i^p]$
       \STATE Set $\nu^r_{i,k}(x)=0$ for all $i\in[\ell]$ and $x\in \cX[Z_i^r]$
       \STATE \texttt{continue} = \textsf{True}
       \WHILE{\texttt{continue}}
            \STATE Observe the current state $s_{t}$, play action $a_t=\pi_{k}^+(s_t)$, and observe reward $r_t = (r_t[1], \ldots, r_t[\ell])$. Set $x_t=(s_t,a_t)$
            \STATE Set
            $
            \begin{cases}
            \nu^p_{i,k}(x_t[Z^p_i])=\nu^p_{i,k}(x_t[Z^p_i])+1, \quad i\in[m] \\
            \nu^r_{i,k}(x_t[Z^r_i])=\nu^r_{i,k}(x_t[Z^r_i])+1, \quad i\in[\ell] 
            \end{cases}
            $
           % \STATE For all $i\in [m]$, set $\nu^p_{i,k}(x_t[Z^p_i])=\nu^p_{i,k}(x_t[Z^p_i])+1$
           % \STATE For all $i\in [\ell]$, set $\nu^r_{i,k}(x_t[Z^r_i])=\nu^r_{i,k}(x_t[Z^r_i])+1$
            \STATE $\texttt{continue} = \bigwedge_{i\in [m]} \big(\nu^r_{i,k}(x_t[Z^r_i])< N^r_{i,t_k}(x_t[Z^r_i]\big) \wedge \bigwedge_{i\in [\ell]} \big(\nu^p_{i,k}(x_t[Z^p_i])< N^p_{i,t_k}(x_t[Z^p_i]\big) $
            \STATE Set $t=t+1$
       \ENDWHILE
        \STATE Set
        $
        \!\begin{cases}\!
        N^p_{i,t_k}(x)\!=\!N^p_{i,t_{k-1}}(x)\!+\!\nu^p_{i,k-1}(x), \, i\!\in\![m],x\!\in\!\cX[Z_i^p] \\
        N^r_{i,t_k}(x)\!=\!N^r_{i,t_{k-1}}(x)\!+\!\nu^r_{i,k-1}(x), \, i\!\in\![\ell],x\!\in\!\cX[Z_i^r] 
        \end{cases}
        $
   \ENDFOR
\end{algorithmic}
\normalsize
\end{algorithm}
%
%\begin{algorithm}[!hbtp]	
%	\caption{\EVI$(c, \cC, \epsilon)$}
%	\label{alg:EVI}
%    \footnotesize
%\begin{algorithmic}
%		%\REQUIRE $\epsilon_t$
%		\STATE Let $u_0\equiv 0, u_{-1}\equiv-\infty$, $n=0$
%		\WHILE{$\bS(u_{n}-u_{n-1}) > \epsilon$}
%		\STATE $\!\!\!$Compute
%		$\begin{cases}
%	 \mu^+: x\mapsto\max \{\mu':  \mu' \!\in\! c_{t,\delta}(x)\}\\
%		P^+_{n}: x\mapsto \argmax \{ \sum_{y\in \cS} P'(y)u_n(y):  P'\!\in\! \cC(x)\}		
%		\end{cases}$
%		\STATE Compute $P^+_{n}(\cdot|x) = \texttt{InnerMaximization}(u_n, \cC(x))$ -- See Algorithm \ref{alg:InMax} in the supplementary. 
%		\STATE $\!\!\!$Update
%	$\!\begin{cases}
%\!u_{n+1}\!(s) =   \max\{ \mu^+\!(s,a) \!+\! \sum_{y\in \cS} P^+_n(y|s,a)u_n(y)\!\!: {a\!\in\!\!\cA}\}\\
%\!\pi^+_{n+1}\!(s) \!\in\! \Argmax\{\mu^+\!(s,a) \!+\! \sum_{y\in \cS} P^+_n(y|s,a)u_n(y)\!\!:{a\!\in\!\!\cA}\}
%		\end{cases}$
%		\STATE $\!\!\!n=n+1$
%\ENDWHILE
%	\end{algorithmic}
%\normalsize
%\end{algorithm}


\begin{algorithm}[!hbtp]	
	\caption{\EVI$(c, \cC, \epsilon)$}
	\label{alg:EVI}
    \footnotesize
\begin{algorithmic}
	%\REQUIRE $\epsilon_t$
		\STATE Let $u_0\equiv 0, u_{-1}\equiv-\infty$, $n=0$
		\WHILE{$\max_s (u_{n}(s)-u_{n-1}(s)) -\min_s(u_{n}(s)-u_{n-1}(s)) > \epsilon$}
		\STATE $\!\!\!$Compute
		$\begin{cases}
	 \tilde\mu(x)=\max\{\mu':  \mu' \!\in\! c_{t,\delta}(x)\}, \,\forall x\\
	 \widetilde P_{n}(\cdot|x) = \texttt{InnerMax}(u_n, \cC(x)), \,\forall x
		\end{cases}$
%		\STATE Compute $\tilde\mu(x)=\max\{\mu':  \mu' \!\in\! c_{t,\delta}(x)\}$ for all $x$
%		\STATE Compute $\widetilde P_{n}(\cdot|x) = \texttt{InnerMax}(u_n, \cC(x))$ for all $x$-- See Algorithm \ref{alg:InMax}. 
		\STATE $\!\!\!$Update
%	$\!\begin{cases}
%\!u_{n+1}\!(s) =   \max\{ \mu^+\!(s,a) \!+\! \sum_{y\in \cS} P^+_n(y|s,a)u_n(y)\!\!: {a\!\in\!\!\cA}\}\\
%\!\pi^+_{n+1}\!(s) \!\in\! \Argmax\{\mu^+\!(s,a) \!+\! \sum_{y\in \cS} P^+_n(y|s,a)u_n(y)\!\!:{a\!\in\!\!\cA}\}
%		\end{cases}$
		$\!\begin{cases}
\!u_{n+1}\!(s) =   \max_{a\in \cA}\!\Big(\!\tilde\mu(s,a) \!+\! \sum_{y\in \cS}\!\widetilde P_n(y|s,a)u_n(y)\!\Big)\\
\!\pi^+_{n+1}\!(s) \!\in\! \argmax_{a\in \cA}\!\Big(\!\tilde\mu(s,a) \!+\! \sum_{y\in \cS}\!\widetilde P_n(y|s,a)u_n(y)\!\Big)
		\end{cases}$
		\STATE $\!\!\!n=n+1$
\ENDWHILE
	\end{algorithmic}
\normalsize
\end{algorithm}


\begin{algorithm}[!hbtp]	
	\caption{\texttt{InnerMax}$(u, \cC)$}
	\label{alg:InMax}
    \footnotesize
\begin{algorithmic}
		\STATE Let $\cS=\{s_1,s_2,\ldots,s_S\}$ such that $u(s_1)\geq \ldots \geq u(s_{S})$
		\STATE Compute $\!\begin{cases}
P_i^+(y[i])\in \max\{q(y[i]): q\in \cC\}, \quad i\in[m]\\
P_i^-(y[i])\in \min\{q(y[i]): q\in \cC\}, \quad i\in[m]
		\end{cases}$
		\STATE Set 		
	$\!\begin{cases}
P^+(y) = \prod_{i=1}^m P^+_i(y[i])\\
		P^-(y) = \prod_{i=1}^m P^-_i(y[i])
		\end{cases}$		
		\STATE For $j\in [S]$, set $q(s_j) = \prod_{i=1}^m P_i^-(s_j[i])$
		\STATE $l = 1$
\WHILE{$\sum_{j=1}^S q(s_j) > 1$ and $l\leq S$}
			\STATE $q' = \prod_{i=1}^m P_i^{+}(s_l[i])$ 
			\STATE $q(s_l)\!=\!\max\Big(q(l)\!+\!\min\Big(1\!-\!\sum_{j=1}^S q(s_j), q'\!-\!q(s_l)\Big), 1\Big)$
			\STATE $l = l + 1$
\ENDWHILE
	\end{algorithmic}
\normalsize
\end{algorithm}

==> sections/background_arXiv.tex <==
%\vspace{-2mm}\noindent
%\section{FACTORED MODEL AND PROBLEM FORMULATION}\label{sec:model}
\section{Problem Formulation}\label{sec:model}
%\vspace{-2mm}\noindent
We study a learning task in a finite MDP $M = (\cS, \cA, P, R)$ under the average-reward criterion, where $\cS$ denotes the set of states with cardinality $S$, $\cA$ denotes the set of actions (available at each state) with cardinality $A$, and $P$ and $R$ denote the transition and reward functions, respectively. Choosing action $a\in \cA$ in state $s\in \cS$ results in a transition to a state $s'\sim P(\cdot|s,a)$ and a reward drawn from $R(s,a)$, with mean $\mu(s,a)$. In the rest of this section, we formally introduce the setup, and present some necessary notations and definitions. 


%\vspace{-2mm}\noindent
\paragraph{Factored Representations}
We assume that $M$ is an FMDP, namely its transition and reward functions admit some conditional independence structure. To formally describe the factored structure, we introduce a few notations and definitions that are standard in the literature on FMDPs (see, e.g., \cite{szita2009optimistic,osband2014near}). We begin by introducing the \emph{scope} operator for a factored set. % We assume that $\cX$ has a factored form: $\cX = \cX_1\times \cdots \cX_n$. 
%\vspace{-2mm}\noindent
\begin{definition}[{Scope Operator for a Factored Set $\cX$}]
Let $\cX\!=\!\otimes_{i=1}^n \cX_i$ be a finite factored set. For any subset of indices $Z\!\subseteq \![n]$, we define $\cX[Z]\!:=\! \otimes_{i\in Z} \cX_i$. Moreover, for any $x\!\in\! \cX$, we let $x[Z] \!\in\! \cX[Z]$ denote the value of the variables $x_i\!\in\! \cX_i$ with indices $i\!\in\! Z$. For $i\!\in\! [n]$, we will write $x[i]$ as a shorthand for $x[\{i\}]$. 
\end{definition}


%\vspace{-1mm}\noindent
An FMDP is represented by a tuple 
$$
M = \big(\{\cS_i\}_{i\in [m]}, \{\cX_i\}_{i\in [n]}, \{P_i\}_{i\in [m]}, \{Z_i^p\}_{i\in [m]}, \{R_i\}_{i\in [\ell]},\{Z_i^r\}_{i\in [\ell]}\big)\, ,
$$
where $\cS_i$ is a state factor, $\cX_i$ is a state-action factor, $P_i$ is the transition function associated with $\cS_i$, $R_i$ is the $i$-th reward function, and $Z_i^p$ (resp.~$Z_i^r$) denotes the scope set of $P_i$ (resp.~$R_i$) for $\cX=\otimes_{i=1}^n \cX_i$. The state-space is $\cS = \otimes_{i=1}^m \cS_i$ and the state-action space is $\cX=\cS_1\otimes\cdots\otimes\cS_m\otimes\cA_1\otimes\cdots\otimes\cA_{n-m} = \cS\times\cA$, where $\cA=\cA_1\otimes\cdots\otimes\cA_{n-m}$ is the (possibly factored) action space\footnote{Some authors have studied compact representations of the state-action space, such as decision trees, but we do not consider this setting in the present paper.}. Given sets $\cX$ and $\cS$, let $\cR_{\cX,[0,1]}$ be the set of all reward functions on $\cX$ with image bounded in $[0,1]$,
%\footnote{Without loss of generality, we consider rewards supported on $[0,1]$.} 
\footnote{Without loss of generality, we consider rewards in $[0,1]$.} 
and let $\cP_{\cX,\cS}$ be the set of all transition functions from $\cX$ to $\cS$, i.e.~each $P\in\cP_{\cX,\cS}$ has one element $P(s|x)\geq 0$ for each $(x,s)\in\cX\times\cS$ and satisfies $\sum_{s\in\cS}P(s|x)=1$ for each $x\in\cX$.
%\vspace{-2mm}\noindent
\begin{definition}[{Factored Reward Functions}]
The class $\cR$ of reward functions is factored over $\cX\!=\!\otimes_{i=1}^n \cX_i$ with scopes $Z_1^r,\ldots,Z_\ell^r$ if and only if for all $R\!\in\! \cR$ and $x\!\in\! \cX$, there exist $\{R_i\!\in\! \cR_{\cX[Z_i^r],[0,1]}\}_{i\in [\ell]}$ such that 
any realization $r\sim R(x)$ implies $r=\sum_{i=1}^\ell r[i]$ with $r[i]\sim R_i(x[Z_i^r])$. Furthermore, let us define $r^{\text{col}}= \tfrac{1}{\ell}\sum_{i=1}^\ell r[i]$. 
%We further let $\cR_{\cX,\cS}^{\textrm{fac}}(Z_1^R,\ldots,Z_l^R) = \otimes_{i=1}^l \cR_{\cX[Z_i], [0,1]}$.  
\end{definition}

%\vspace{-2mm}\noindent
\begin{definition}[{Factored Transition Functions}]
The class $\cP$ of transition functions is factored over $\cX=\otimes_{i=1}^n \cX_i$ and $\cS = \otimes_{i=1}^m \cS_i$ with scopes $Z_1^p,\ldots,Z_m^p$ if and only if for all $P\in \cP$ and $x\in \cX$ and $s\in \cS$, there exist $\{P_i\in \cP_{\cX[Z_i^p], \cS_i}\}_{i\in [m]}$ such that 
$
P(s|x) = \prod_{i=1}^m P_i\big(s[i]\big|x[Z_i^p]\big) \, .
$
%We further let $\cP_{\cX,\cS}^{\textrm{fac}}(Z_1^P,\ldots,Z_m^P) = \otimes_{i=1}^m \cP_{\cX[Z_i], \cS_i}$.  
\end{definition}

%\vspace{-2mm}\noindent
In order to clarify the presentation of confidence sets in the subsequent sections, we further introduce the following more compact representation of a FMDP. Let $\cG_r = \big(\{\cX_i\}_{i\in [n]}; \{Z_i^r\}_{i\in [\ell]}\big)$ and $\cG_p = \big(\{\cX_i\}_{i\in [n]}, \{\cS_i\}_{i\in [m]}; \{Z_i^p\}_{i\in [m]}\big)$. We compactly represent a FMDP with structure $\cG= \cG_r \cup \cG_p$ by a tuple
$M = \big(\{P_i\}_{i\in [m]}, \{R_i\}_{i\in [\ell]}; \cG\big),$
and let $\cG(M)$  denotes its  corresponding structure. We finally introduce the set $\mathbb{M}_\cG$ of all FMDPs with structure  $\cG$: 
$$
\mathbb M_{\cG}\!=\!\Big\{M\!=\!(P,\!R;\!\cG)\!:\! P\!\in\!\cP_{\cX,\cS}^{\textrm{fac}}(\cG_p) \hbox{ and }  R\!\in\!\cR_{\cX,[0,1]}^{\textrm{fac}}(\cG_r)\Big\}\, ,
$$
where $\cP_{\cX,\cS}^{\textrm{fac}}(\cG_p) = \otimes_{i=1}^m \cP_{\cX[Z_i^p], \cS_i}$ and $\cR_{\cX,[0,1]}^{\textrm{fac}}(\cG_r) = \otimes_{i=1}^\ell \cR_{\cX[Z_i^r], [0,1]}$. 

%\vspace{-1mm}\noindent
\begin{remark}
An FMDP $M$ can be represented by a Dynamic Bayesian Network (DBN) $\cB=(\cV,\cE,\cT)$, where $\cV$ is a set of $m$ discrete variables $\{v_i\}_{i\in[m]}$ and $\ell$ continuous variables $\{u_j\}_{j\in[\ell]}$, duplicated on two timeslices, $\cE$ is a set of edges between the two timeslices, and $\cT$ is a set of conditional probability tables (CPTs). In this case, $\cS_i = \cD(v_i)$ is the domain of variable $v_i$, $i\in[m]$, $\cX[Z_i^p]$ (resp.~$\cX[Z_j^r]$) are the elements used to index the rows of the CPT of variable $v_i$ (resp.~$u_j$), and $\cX[Z_i^p]$ (resp.~$\cX[Z_j^r]$) distinguishes between elements of $\cS_k$, $k\in[m]$, if and only if $(v_k,v_i)\in\cE$ (resp.~$(v_k,u_j)\in\cE$). In this context, $\cG$ is the structure of the DBN $\cB$ while $P$ and $R$ are the parameters of the CPTs in $\cT$. By a slight abuse of terminology, we refer to $\cG(M)$ as the DBN structure of FMDP $M$. 
\end{remark}

%\vspace{-2mm}\noindent
\paragraph{Regret Minimization in FMDPs}
We consider a finite FMDP $M = \big(\{P_i\}_{i\in [m]}, \{R_i\}_{i\in [\ell]}; \cG\big)$ and the following RL task. An agent interacts with $M$ for $T$ rounds, starting in an initial state $s_1\in \cS$ chosen by Nature. At each time $t$, the agent is in state $s_t = (s_t[1],\ldots,s_t[m])$ and chooses an action $a_t$ based on her observations so far. Let $x_t=(s_t,a_t)$ denote the state-action pair of the agent at time $t$. Then, (i) she receives a reward vector $r_t = (r_t[1],\ldots, r_t[\ell])$, where for each $i\in [\ell]$, $r_t[i]\sim R_i(x_t[Z_i^r])$; and (ii) Nature decides a next state $s_{t+1} = (s_{t+1}[1],\ldots,s_{t+1}[m])$ where for each $i\in [m]$, $s_{t+1}[i]\sim P_i(\cdot|x_t[Z_i^p])$. Let $r^{\text{col}}_t = \tfrac{1}{\ell} \sum_{i\in [\ell]} r_t[i]$ denote the normalized collected reward at time $t$. 

The goal of the agent is to maximize the cumulative reward $\sum_{t=1}^T r^{\text{col}}_t = \sum_{t=1}^T \tfrac{1}{\ell} \sum_{i\in [\ell]} r_t[i]$, where $T$ denotes the time horizon. We assume that the agent perfectly knows $\cG$, but not the transition function $P$ and reward function $R$. She therefore has to learn them by trying different actions and recording the realized rewards and state transitions. The performance of the agent can be assessed resorting to the notion of regret. Following \cite{jaksch2010near}, we define the regret of a learning algorithm $\mathbb A$, after $T$ steps and starting from an initial state $s_1\!\in\! \cS$, as:
%\vspace{-2mm}\noindent
\als{
\kR(T, \mathbb A, s_1) = Tg^\star(s_1) - \sum_{t=1}^T r^{\text{col}}_t \, ,
}
%\vspace{-2mm}\noindent
where $g^\star$ denotes the long-term average-reward (or gain) of the MDP starting from state $s_1$; we refer to \citep{puterman2014markov} for further details. Alternatively, the objective of the agent is to minimize the regret, which calls for balancing exploration and exploitation.
In this paper we consider communicating MDPs, for which the gain does not depend on $s_1$, that is, $g^\star(s_1) \!=\! g^\star$ for all $s_1\!\in\! \cS$. We therefore define: $\kR(T, \mathbb A) = Tg^\star \!- \!\sum_{t=1}^T  r^{\text{col}}_t$. The class of communicating MDPs arguably captures a big class of RL tasks of practical interest, and most literature on regret minimization in the average-reward setting has developed algorithms for this class. A notable property of communicating MDPs is having a finite {\it diameter}, as formalized in \citep{jaksch2010near}\footnote{Given an MDP $M$, the diameter $D := D(M)$ is defined as $D(M) := \max_{s\neq s'} \min_{\pi:\cS\to \cA} \EE[T^\pi (s,s')]$, where $T^\pi (s,s')$
denotes the number of steps it takes to get to $s'$ starting from $s$ and following policy $\pi$ \citep{jaksch2010near}.}. 






%{\color{blue}
%\paragraph{Notations.} We introduce some notations that will be used throughout.  For a distribution $p\in\Delta_\cS$ and a vector-function $f = (f(s))_{s\in\cS}$, we denote $Pf$ its application $f$, defined by $Pf=\Esp_{S\sim p}[f(S)]$. Likewise, for $p\in\Delta_\cS^{\cS\times\cA}$, we define the corresponding operator $P$ such that $Pf: s,a\mapsto  \Esp_{S\sim p(\cdot|s,a)}[f(S)]$.
%We also introduce $\bS(f) = \max_s f(s) - \min_s f(s)$. For $x\in \RR$, we let $x^+ := \max\{x,1\}$. 
%%Under a given algorithm and for a pair $(s,a)$, we denote by $N_t(s,a)$ the total number of observations of $(s,a)$ up to time $t$. Let us define $\widehat \mu_{t}(s,a)$ as the empirical mean reward built using $N_t(s,a)$ i.i.d.~samples from $\nu(s,a)$, and $\widehat p_t(\cdot|s,a)$ as the empirical distribution built using $N_t(s,a)$ i.i.d.~observations from $p(\cdot|s,a)$.
%}



==> sections/factorization_lemma_proof_arXiv.tex <==

\section{A Factorization Lemma (Proof of Lemma \ref{lem:factored_deviation})}
\label{app:proof_factorization_lemma}


In this section, we prove Theorem \ref{thm:regret_Alg1}. Before presenting the proof, we collect some necessary lemmas. The first one, which plays a crucial role in the proof, presents a bound on factored deviations, and can be seen as a refined variant of Lemma 1 in \cite{osband2014near}. 

\begin{lemma}
\label{lem:factored_deviation}
Let $P$ and $P'$ be two probability measures defined over $\cS=\cS_1\times\cdots\times \cS_m$ such that for all $y=(y_1,\ldots,y_m)\in \cS$: $P(y)=\prod_{i=1}^m P_i(y_i)$ and $P'(y)=\prod_{i=1}^m P'_i(y_i)$. Assume that for all $i\in [m]$, there exist $\xi_i,\xi'_i>0$ such that 
$$
|(P'_i-P_i)(y_i)|\leq \sqrt{P_i(y_i)\xi_i} + \xi'_i\, , \quad \forall y_i\in \cS_i.
$$
Then, for any function $f:\cS\to \RR_+$, we have
\als{
\sum_{y\in \cS} |(P-P')(y)|f(y) &\leq \max_{y\in\otimes_{i=1}^m\supp(P_i)} f(y) \sum_{i=1}^m \sum_{y_i\in\cS_i}\sqrt{P_i(y_i)\xi_i} + 3\max_{y\in \cS} f(y)\sum_{i=1}^m \xi'_iS_i\, .
}
\end{lemma}

\bp
We prove the lemma by induction on $m$. 
For the case of $m=2$, we have
\als{
\sum_{y\in \cS} |(P-P')(y)|f(y) &\leq \sum_{y_1}\sum_{y_2} |P_1(y_1)P_2(y_2) - P'_1(y_1)P'_2(y_2)|f(y) \\
&\leq \sum_{y_1}\sum_{y_2} P_1(y_1)|P_2(y_2) - P'_2(y_2)| f(y)\\
&+ \sum_{y_1}\sum_{y_2} P'_2(y_2)|P_1(y_1) - P'_1(y_1)| f(y) \, .
}
The first term is bounded as:
\als{
\sum_{y_1}\sum_{y_2} P_1(y_1)|P_2(y_2) &- P'_2(y_2)| f(y) \leq  \sum_{y_2} |P_2(y_2) - P'_2(y_2)| \max_{y_1\in \supp(P_1)} f(y)\underbrace{\sum_{y_1} P_1(y_1)}_{=1} \\
&\leq  \sum_{y_2} \max_{y_1\in \supp(P_1)} f(y)\Big(\sqrt{P_2(y_2)\xi_2} + \xi'_2\Big) \\
&\leq \max_{y_1\in \supp(P_1),y_2\in\supp(P_2)} f(y) \sum_{y_2} \sqrt{P_2(y_2)\xi_2} + \xi'_2 S_2\max_y f(y) \, .
}
For the second term we get:
\als{
\sum_{y_1}\sum_{y_2} P'_2(y_2)|P_1(y_1) &- P'_1(y_1)| f(y)  \\
&\leq \sum_{y_1}|P_1(y_1) - P'_1(y_1)| \bigg(\sum_{y_2\in \mathrm{supp}(P_2)} P'_2(y_2)f(y) 
+ \sum_{y_2\notin \mathrm{supp}(P_2)} P'_2(y_2)f(y) \bigg)\\
&\leq \sum_{y_1}|P_1(y_1) - P'_1(y_1)| \Big(\max_{y_2\in\supp(P_2)} f(y) \sum_{y_2\in \mathrm{supp}(P_2)} P'_2(y_2) 
+ \max_{y}f(y) \sum_{y_2\notin \mathrm{supp}(P_2)} P'_2(y_2)\Big)\\
&\leq \sum_{y_1}|P_1(y_1) - P'_1(y_1)| \Big(\max_{y_2\in\supp(P_2)} f(y)
+ \xi'_2S_2\max_{y}f(y)\Big)\\
&\leq \sum_{y_1} \sqrt{P_1(y_1)\xi_1} \max_{y_2\in\supp(P_2)} f(y) + 2\xi'_2S_2\max_{y}f(y)  \\
&\leq \max_{y_1\in \supp(P_1),y_2\in\supp(P_2)} f(y) \sum_{y_1} \sqrt{P_1(y_1)\xi_1} + 2\xi'_2S_2\max_{y}f(y)  \,,
}
where we used $\sum_{y_1} |(P_1 - P'_1)(y_1)| \leq 2$. Hence,
\als{
\sum_{y\in \cS} (P-P')(y)f(y) &\leq \max_{y_i\in \otimes_{i=1}^2\supp(P_i)} f(y)  \sum_{i=1}^2\sum_{y_i} \sqrt{P_i(y_i)\xi_i} + 3\max_{y}f(y) \sum_{i=1}^2 \xi'_iS_i\, .
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% \sadegh{It would suffice to choose 2 instead of 3 above.}

Now assume that the induction hypothesis is correct for $m>2$:
\als{
\sum_{y\in \cS} |(P-P')(y)|f(y)  &\leq \max_{y_i\in \otimes_{i=1}^m\supp(P_i)} f(y)  \sum_{i=1}^m\sum_{y_i} \sqrt{P_i(y_i)\xi_i} + 3\max_{y}f(y) \sum_{i=1}^m \xi'_iS_i\, .
}
We then show that the above holds for $m+1$. To this aim, let $P(y) = q(y_{1:m})P_{m+1}(y_{m+1})$ and  $P'(y) = q'(y_{1:m})P'_{m+1}(y_{m+1})$, where we defined the short-hand $y_{1:m} := y_1,\ldots,y_{m}$. 
We have:
\als{
\sum_{y} (P-P')(y)f(y) &\leq \sum_{y} \Big|P_{m+1}(y_{m+1})q(y_{1:m}) - P'_{m+1}(y_{m+1})q'(y_{1:m})\Big|\, \big|f(y)\big| \\ 
&\leq \sum_{y_{1:m}}\sum_{y_{m+1}} q(y_{1:m})|(P_{m+1} - P'_{m+1})(y_{m+1})| f(y)  \\ 
&+\sum_{y_{m+1}}\sum_{y_{1:m}} P'_{m+1}(y_{m+1})|(q - q')(y_{1:m})| f(y) \, .
}
The first term is bounded as:
\al{
\sum_{y_{m+1}}&\sum_{y_{1:m}} q(y_{1:m})|(P_{m+1} - P'_{m+1})(y_{m+1})| f(y)  \sk
&\leq  \sum_{y_{m+1}} |(P_{m+1} - P'_{m+1})(y_{m+1})| \max_{y_{1:m}\in \otimes_{i=1}^{m} \mathrm{supp}(P_i)} f(y)  \underbrace{\sum_{y_{1:m}} q(y_{1:m})}_{=1} \sk
&\leq  \sum_{y_{m+1}} \Big(\sqrt{P_{m+1}(y_{m+1})\xi_{m+1}} + \xi'_{m+1}\Big) \max_{y_{1:m}\in \otimes_{i=1}^m \mathrm{supp}(P_i)} f(y)  \sk
\label{eq:1st_term}
&\leq  \max_{y\in \otimes_{i=1}^{m+1} \mathrm{supp}(P_i)} f(y)  \sum_{y_{m+1}} \sqrt{P_{m+1}(y_{m+1})\xi_{m+1}} + \xi'_{m+1}S_{m+1} \max_y f(y) 
 \, .
}
The second term is bounded as follows:
\al{
&\sum_{y_{m+1}}\sum_{y_{1:m}} P'_{m+1}(y_{m+1})|(q - q')(y_{1:m})| f(y)   \sk
&\leq \sum_{y_{1:m}} |(q - q')(y_{1:m})|  \Big(\sum_{y_{m+1}\in \mathrm{supp}(P_{m+1})} P'_{m+1}(y_{m+1})f(y)  
+ \sum_{y_{m+1}\notin \mathrm{supp}(P_{m+1})} P'_{m+1}(y_{m+1})f(y) \Big)\sk
\label{eq:2nd_term}
&\leq \sum_{y_{1:m}}|(q - q')(y_{1:m})| \max_{y_{m+1}\in \mathrm{supp}(P_{m+1})} f(y) 
+ 2\xi'_{m+1}S_{m+1}\max_{y} f(y)  \,.
}
Note that the induction hypothesis implies 
\als{
\sum_{y_{1:m}}|(q - q')(y_{1:m})| \max_{y_{m+1}\in \mathrm{supp}(P_{m+1})} f(y)  &\leq \max_{y_i\in \otimes_{i=1}^{m+1}\supp(P_i)} f(y)  \sum_{i=1}^{m}\sum_{y_i} \sqrt{P_i(y_i)\xi_i} 
\\
&+ 3\max_{y}f(y) \sum_{i=1}^m \xi'_iS_i\, .
}
Putting this together with (\ref{eq:2nd_term}), and combining with (\ref{eq:1st_term}) yield the desired result:
\als{
\sum_{y} |(P-P')(y)|f(y) &\leq \max_{y_i\in \otimes_{i=1}^{m+1}\supp(P_i)} f(y)  \sum_{i=1}^{m+1}\sum_{y_i} \sqrt{P_i(y_i)\xi_i} + 3\max_{y}f(y) \sum_{i=1}^{m+1} \xi'_iS_i\, ,
}
thus concluding the proof. 
\ep


==> sections/regret_bounds_arXiv.tex <==

%\vspace{-2mm}\noindent
\section{\AlgB: Regret Analysis}\label{sec:results}
%\vspace{-2mm}\noindent
In this section, we present high-probability and finite-time regret upper bounds for \AlgB. Our main result, presented in Theorem~\ref{thm:regret_Alg1}, is a regret upper bound %for \AlgB\ 
assuming a generic structure $\cG$. It is followed by Theorem \ref{thm:regret_Alg1_Cartesian} stating a substantially refined bound when the underlying structure $\cG$ admits a Cartesian product form. Before presenting the regret bounds, we introduce a new notion of diameter in FMDPs. 


\paragraph{Factored Diameter}
The regret bound of Theorem \ref{thm:regret_Alg1} relates the regret to a new notion of connectivity in FDMPs presented below. 
%\begin{definition}[Factored Diameter]
%The \emph{factored diameter} of an FMDP $M$ for $i\!\in\! [m]$ and at state $y\!\in\! \cS[Z_i^p]$, denoted by $D_{i,y}:=D_{i,y}(M)$ is defined as
%\als{
%D_{i,y} = \max_{s'\in \cS: s'[Z^p_i] = y} \max_{s_1,s_2\in \cL_{i,s'}} \min_\pi \EE[T^\pi(s_1,s_2)]\, ,
%}

\begin{definition}[Factored Diameter]
\label{def:factored_diameter}
The \emph{factored diameter} of an FMDP $M$ for $u\in \cS[Z_i^p]$ along factor $i\in[m]$, denoted by $D_{i,u}=D_{i,u}(M)$, is defined as
\als{
D_{i,u} = \max_{s\in \cS: s[Z^p_i] = u} \max_{s_1,s_2\in \cL_{s}} \min_\pi \EE[T^\pi(s_1,s_2)]\, ,
}
where $\cL_{s} := \otimes_{i=1}^m(\cup_{a\in \cA[Z^p_i]} \cK_{i, s[Z_i^p], a})$, and where for $s_1,s_2$ with $s_1\neq s_2$, $T^\pi(s_1,s_2)$ denotes the number of steps it takes to reach $s_2$ starting from $s_1$ by following policy $\pi$. 
\end{definition}
%\vspace{-2mm}


\begin{figure}[!t]
\begin{center}
	\includegraphics[scale=.85]{images/MDP_diameter.pdf}
    \caption{Global vs.~Factored Diameter}
 	\label{fig:diameter}
\end{center}
\end{figure}

The notion of factored diameter refines that of diameter $D$ of \citep{jaksch2010near} (we refer to Section \ref{sec:model}), and extends the notion of local diameter in \citep{bourel2020tightening} for tabular MDPs to FMDPs, in the sense that in the absence of factorization (i.e., when the DBN is a complete graph), the factored diameter coincides with the local diameter in \citep{bourel2020tightening}. The factored diameter takes into account the joint support sets of factors, and is therefore a problem-dependent refinement of the global diameter $D$. 
In particular, for all $i$ and $u\in \cS[Z_i^p]$, $D_{i,u} \le D$. Interestingly, there exist cases where $D_{i,y} \ll D$, as we illustrate through an example below, which is motivated by a multi-agent RL scenario. 

Consider $2$ agents, each independently interacting with an instance of the $n$-state MDP shown in Figure \ref{fig:diameter}. %The action-space is state-dependent: in all state $s\neq (s_{n-1},s_{n-1})$, $\cA_s=\{a,b\}$, whereas in $\cA_{s_{n-1}} =\{b\}$. 
Each agent $i\in\{1,2\}$ occupies a state in $\cS_i=\{s_1,s_2,\ldots,s_n\}$ with $n>2$, and the transition function $P_i$ is defined according to the MDP shown in the figure.
%Consider this MDP showing interaction of $2$ agents with an environment. The states of agents evolve independently of each other, but each follows an MDP as shown in Figure \ref{fig:diameter}: Each   
In each state $s\neq s_{n-1}$, each agent has access to two actions $a$ and $b$. Only when both agents are \emph{simultaneously} in $s_{n-1}$, they have access to an extra action $a'$, which causes each agent to stochastically (but independently) transit to a high-reward state $s_n$ --- For instance, this could be relevant in scenarios where cooperation yields higher rewards. 
This scenario can be modeled using an FMDP as follows. The state-space is $\cS=\cS_1\times \cS_2$ and the action-space is state-dependent: in each state $s\neq (s_{n-1},s_{n-1})$, $\cA_s=\{a,b\}\times \{a,b\}$, whereas in $s=(s_{n-1},s_{n-1})$, $\cA_s =\{a',b\} \times \{a',b\}$. 

For the case of a single agent, observe that $D=\frac{n-1}{\delta}$, as it takes $\frac{n-1}{\delta}$ steps in expectations to reach $s_n$ from $s_1$ (the worst-case travel time). % $D'=2/\delta$, which is the worst-case shortest path between any pair of states in the support of any state. 
In the considered FMDP, it is easy to verify that $D=\big(\tfrac{n-1}{\delta}\big)^2$. The factored diameter here is at most $\tfrac{4}{\delta^2}$. Indeed, for $s=(s_i,s_j)$, we have $\cL_{s} = \{s_{(i-1)\vee 1},s_{i},s_{(i+1)\wedge n}\}\times\{s_{(j-1)\vee 1},s_{j},s_{(j+1)\wedge n}\}$,\footnote{We use shorthands $a\vee b\!=\!\max\{a,b\}$ and $a\wedge b\!=\!\min\{a,b\}$.} and one can verify that for any two states $u,v\in \cL_s$, it takes at most  $\tfrac{4}{\delta^2}$ steps in expectation to reach $u$ starting from $v$ -- For details see Appendix \ref{app:diameter}.

In this example, the factored diameter is smaller than $D$ by a factor of $\cO(n^2)$. Now, if we extend this to the case of $m$ agents, the ratio of $D$ and the factored diameter would be $\cO(n^m)$. This further implies that \AlgB\ achieves a much tighter regret than DORL and UCRL-Factored in these cases. Let us remark that such a massive reduction is a consequence of using Bernstein-type concentration inequalities for transition function that takes into account the support of $P_i$. We however stress that in contrast to non-fatored MDPs where a corresponding local diameter is straightforward to define (as done in \citep{bourel2020tightening}), the task in FMDPs involves technical challenges for the decomposition of transition function along factors. To carefully exploit the gain of using Bernstein confidence intervals for $P_i$, we rely on the following factored deviation lemma, which can be seen as a refined variant of Lemma 1 in \citep{osband2014near}, and whose proof is reported in Appendix \ref{app:proof_factorization_lemma}. :

\begin{lemma}
\label{lem:factored_deviation}
Let $P$ and $P'$ be two probability measures defined over $\cS=\cS_1\times\cdots\times \cS_m$ such that for all $y=(y_1,\ldots,y_m)\in \cS$: $P(y)=\prod_{i=1}^m P_i(y_i)$ and $P'(y)=\prod_{i=1}^m P'_i(y_i)$. Assume that for all $i\in [m]$, there exist $\xi_i,\xi'_i>0$ such that 
$
|(P'_i-P_i)(y_i)|\leq \sqrt{P_i(y_i)\xi_i} + \xi'_i$, for all $y_i\in \cS_i.
$
Then, for any function $f:\cS\to \RR_+$, 
\als{
\sum_{y\in \cS} |(P-P')(y)|f(y) \leq 3\max_{y\in \cS} f(y)\sum_{i=1}^m \xi'_iS_i 
+\max_{y\in\otimes_{i=1}^m\supp(P_i)} f(y) \sum_{i=1}^m \sum_{y_i\in\cS_i}\sqrt{P_i(y_i)\xi_i} \, .
}
\end{lemma}


 




\paragraph{Regret Bound for Generic Structure}Before stating Theorem \ref{thm:regret_Alg1}, let us introduce a few additional quantities. For $i\in [m]$ and $x\in \cX[Z^p_i]$, we define: 
$
\cK_{i,x}:=\supp(P_i(\cdot|x)), \quad K_{i,x} := |\cK_{i,x}|.
$ 

 %We conclude this section by introducing a key problem-dependent quantity capturing the difficulty of learning in an MDP. In average-gain regret minimization, the diameter of an MDP plays a special role.
%The diameter is defined as the maximal value over pairs of states of the minimum expected travel time between these states. We now introduce a 
%factored and local version of this quantity.
%\begin{definition}[Local Diameter of State $s$ \cite{bourel2020tightening}]
%	Consider state $s\in \cS$. For $s_1,s_2\in \cup_{a\in \cA} \supp(p (\cdot|s,a))$ with $s_1\neq s_2$, let $T^\pi(s_1,s_2)$ denote the number of steps it takes to get to $s_2$ starting from $s_1$ and following policy $\pi$. Then, the local diameter of MDP $M$ for $s$, denoted by $D^{\textrm{local}}_{s}:=D^{\textrm{local}}_{s}(M)$ is defined as
%	$$
%	D^{\textrm{local}}_{s}:= \max_{s_1,s_2 \in  \cup_a \supp(p (\cdot|s,a))}   \min_\pi \Esp[T^\pi(s_1,s_2)].
%	$$
%\end{definition}
%\vspace{-2mm}\noindent
\begin{theorem}[Regret of \AlgB]\label{thm:regret_Alg1}
		Uniformly over all $T\ge 3$, with probability higher than $1-\delta$, it holds that
		\als{
			\kR(\mathrm{\AlgB},T) \leq  \cO\bigg( c(M)\sqrt{T \log\big(\log(T)/\delta\big)} 
			+ D(\sum_{i=1}^m |\cX[Z^p_i]| + \sum_{i=1}^\ell |\cX[Z^r_i]|)\log(T)\bigg)\,,
			%&+ 10DKS^{2/3}A^{2/3}T^{1/3} + \cO\Big(DS^2A\log^2\big(\tfrac{T}{\delta}\big)\Big),
		}	
		with 		$c(M)=\sum\nolimits_{i\in [m]}\sqrt{\sum\nolimits_{(s,a)\in\cX[Z^p_i]} D^2_{i,s}(K_{i,s,a}-1)} +\sum\nolimits_{i\in[\ell]} \sqrt{|\cX[Z^r_i]|} + \max_{i,s\in\cS[Z_i^p]} D_{i,s}$. 
%		Therefore, the regret of \AlgB\ asymptotically grows as 
%		$$
%\cO\Big(\sum_{i=1}^m \sum_{x\in \cX[Z_i]} (\ \Big).
%$$		
\end{theorem}

In comparison, the regret of UCRL-Factored and DORL satisfies $\widetilde \cO(D\sum_{i=1}^m \sqrt{S_i |\cX[Z^p_i]|T})$.%, where $D$ denotes the (global) diameter of the FMDP. 
The regret bound of \AlgB\ improves over these regret bounds as for all $i\in [m]$ and $(s,a)\in\cX[Z_i^p]$, we have $K_{i,s,a} \le S_i$ and $D_{i,s}\leq D$. In view of the fact that in some FMDPs $D_{i,s}\ll D$, this improvement can be substantial in some domains. We also demonstrate through numerical experiments on standard environments that \AlgB\ is significantly superior to existing algorithms in terms of practical regret. % We also emphasize that the rewards in the considered FMDP are assumed to be in $[0,\ell]$, and therefore the multiplicative term $\ell$ appears in the leading term there. We note that this point has been overlooked in the regret analysis of DORL in \cite{xu2020near}, and therefore the correct regret bound of DORL would suffer from the same multiplicative factor $\ell$.  
We finally note that \citep{xu2020near} presented another measure called factored span, and present an algorithm following Regal \citep{bartlett2009regal}, whose regret scales with the factored span (and not $D$). However, by design the presented algorithm crucially relies on knowing a priori an upper bound on the factored span. We also add that factored diameter and factored span are not directly comparable. In contrast, the bound in Theorem \ref{thm:regret_Alg1} is valid without any such prior knowledge. 

The proof of Theorem \ref{thm:regret_Alg1} is provided in Appendix \ref{app:regret_proof_generic} in the supplementary material. Similarly to most UCRL2-style algorithms, the proof of this theorem follows the machinery of the regret analysis in \citep{jaksch2010near}. However, to account for the underlying factored structure, as in the regret analyses in (\citet{osband2014near,xu2020near}), the proof decomposes the regret across factors. The algorithms in  \citep{osband2014near,xu2020near} both rely on $L_1$-type confidence sets, as in UCRL2 \citep{jaksch2010near}, and their corresponding regret analyses proceed by decomposing an $L_1$ distance between two probability distributions to the sum of  $L_1$ distances over various factors. This decomposition necessarily involves the global diameter $D$ in the leading term of regret. In contrast, \AlgB\ relies on Lemma \ref{lem:factored_deviation}, which carefully exploits the benefit of using the Bernstein-style confidence sets. %This decomposition lemma proves essential to have a regret bound whose leading term scales as $D_{i,y}$ instead of $D$ (see Lemma \ref{lem:factored_deviation} in Appendix \ref{app:proof_factorization_lemma}). 


\paragraph{Regret Bound for Cartesian Products} 
We now focus on the specific case where the structure $\cG$ can be decomposed to the Cartesian products. 
In this case, the true FMDP $M$ can be seen as the Cartesian products of some base MDPs.  To present the regret bound of \AlgB\ for this case, let the true FMDP $M$ be a Cartesian product of $k$ base MDPs, $M^{(i)}, i=1,\ldots,k$, each with state space $\cS^{i}$, action space 
$\cA^{i}$, and the respective local and global diameters $D^{(i)}_{s}$ and $D^{(i)}$. We have:

%\vspace{-2mm}
\begin{theorem}[Regret of \AlgB\ for Cartesian products]\label{thm:regret_Alg1_Cartesian}

		With probability higher than $1-\delta$, for all $T\ge 3$,
		\als{
			\kR(\mathrm{\AlgB},T) \leq  \cO\bigg( \sum_{i=1}^k c_i\sqrt{T \log\big(\log(T)/\delta\big)} 
			 + \sum_{i=1}^m D^{(i)}S^{(i)}A^{(i)}\log(T)\bigg)\,,
			%&+ 10DKS^{2/3}A^{2/3}T^{1/3} + \cO\Big(DS^2A\log^2\big(\tfrac{T}{\delta}\big)\Big)\,,
		}	
		with 		$c_i=\sqrt{\sum\nolimits_{i\in [k]}\sum\nolimits_{s\in \cS^{(i)}, a\in \cA^{(i)}} \big[D^{(i)}_{s}\big]^2(K^{(i)}_{s,a}-1)} +\sum\nolimits_{i\in[\ell]} \sqrt{S^{(i)}A^{(i)}} + \max_{s\in \cS^{(i)}} D^{(i)}_s$. 
\end{theorem}

%\vspace{-2mm}
The above result asserts that in the case of Cartesian products, the regret of \AlgB\ boils down to the sum of individual regret of $k$ base MDPs, where each individual term corresponds to a fully local quantity, i.e.~depending only on the properties of $M^{(i)}$. This bound significantly improves over previous regret bounds for the product case, which were unable to establish a fully localized regret bound. In particular, the bounds of \cite{osband2014near} and \cite{xu2020near} for this case would necessarily depend on the {\it global diameter of the FMDP} whereas ours in Theorem \ref{thm:regret_Alg1_Cartesian} depends on {\it the local diameter of the local MDPs}. This would in turn imply an exponentially (in the number $k$ of base MDPs) tighter regret bound. 
Finally, we mention that \citep{xu2020near} present a regret lower bound scaling as $\Omega(\sqrt{\mathbf{sp}(h)LT})$ in FMDPs based on worst-case Cartesian products, where $L$ is an upper bound on both $|\cX[Z_i^p]|$ and $|\cX[Z_i^r]|$, and $\mathbf{sp}(h)$ denotes the span of the optimal bias function. Our regret bounds do not contradict this lower bounds as $\mathbf{sp}(h)\le \sum_{i} D_s^{(i)}$ for any $s$.  


\begin{remark}
Cartesian products might seem specific, but admittedly they represent the extreme case of FMDPs, where the individual MDPs are independent of one another. Hence, they are used in existing works (e.g., \cite{osband2014near,xu2020near}) to establish \emph{best-case bounds} on exploration. The resulting bounds are typically more explicit than their corresponding complicated bounds for generic FMDPs. This allowed us to establish a best-case bound depending only in \emph{fully local} quantities, in contrast to existing bounds above for Cartesian products. We believe that there is still value in analysing these special cases, and that analysing intermediate cases (in which individual MDPs are only \emph{weakly connected}) is an important avenue for future work. %This case could be relevant in some application scenarios, as discussed in \cite{lHorincz2016estimating}.
\end{remark}

%For completeness we collect some useful relations from \cite{xu2020near} (see the proof of Lemma E.1 there). We have $g^\star = \sum_{i} g_i^\star$, where $g^\star_i$ denotes the optimal gain of $M_i$. Further, the bias satisfies 
%\als{
%b^\star(s) = \EE[\sum_{t=1}^\infty (r_t - g^\star) | s_1 = s] = \sum_i \EE[\sum_{t=1}^\infty (r_{t}[i] - g^\star_i)| s_1[i] = s[i]] = \sum_{i} b^\star_i(s[i])\, ,
%}
%where for each $i\in[m]$ we define $b_i(s) = \EE[\sum_{t=1}^\infty (r_{t}[i] - g^\star_i)|s_1[i] = s]\, , \forall s\in \cS_i$.  

We finally note that the above result cannot be directly obtained from Theorem \ref{thm:regret_Alg1}, and its proof crucially relies on the following lemma stating that in FMDPs with Cartesian structures, the value function can be decomposed into the sum of individual value functions of the base MDPs:\footnote{A similar results for the bias function of the FMDP in the case of Cartesian product was provided in  \cite{xu2020near}, but not for Value Iteration.} 

\begin{lemma}[Value Iteration for Cartesian products] \label{lem:VI_Cartesian_prod}
Consider VI with $u_0(s) = 0$, and for each $n>1$, $u_{n+1}(s)=\max_{a\in \cA}\big\{r(s,a) + \sum_{y\in \cS} P(y|s,a) u_n(y)\big\}$. Then, $u_{n}(s) = \sum_{i=1}^k u^{(i)}_{n}(s[i])$, where $(u^{(i)}_{n})_{n\geq 0}$ is a sequence of VI on MDP $i$, that is $u^{(i)}_{n+1}(x) = \max_{a\in \cA_i}\big\{r^{(i)}(x,a) +  \sum_{y\in \cS_i} P^{(i)}(y|x,a) u^{(i)}_{n}(y)\big\}$ for all $x\in \cS^{(i)}$ and $n\geq 0$. 
\end{lemma}

%We further note that Cartesian-product FMDPs, \EVI\ can be simply implemented by running \EVI\ on each base MDP independently. We refer to the supplementary for further details. 



==> sections/regret_proofs_arXiv.tex <==

\section{Concentration Inequalities}
\label{app:concentration_inequalities}
In this section, for the sake of completeness, we collect some concentration inequalities used when constructing the set $\cM_{t,\delta}$ of plausible MDPs in \AlgB. The first lemma provides a time-uniform Bernstein-type concentration inequality for bounded random variables: 

\begin{lemma}
\label{lem:Bernstein_peeling}
  Let $Z = (Z_t)_{t\in \NN}$ be a sequence of random  variables generated by a predictable process, and $\cF=(\cF_t)_{t}$ be its natural filtration. Assume for all $t\in \NN$, $|Z_t|\le b$ and $\EE[Z_{s}^2|\cF_{s-1}] \le v$ for some positive numbers $v$ and $b$.
  Let $n$ be an integer-valued (and possibly unbounded) random variable that is $\cF$-measurable. Then, for all $\delta\in (0,1)$,
  \als{
\PP\bigg[\exists n\in \NN, \,\, \frac{1}{n}\sum_{t=1}^{n}Z_t
\geq \sqrt{\frac{2\beta_n(\delta) v}{n}} +  \frac{\beta_n(\delta)b}{3n} \bigg] &\leq \delta\, , \\
\PP\bigg[\exists n\in \NN, \,\, \frac{1}{n}\sum_{t=1}^{n}Z_t \leq -\sqrt{\frac{2\beta_n(\delta) v}{n}} -  \frac{\beta_n(\delta)b}{3n} \bigg]  &\leq \delta\,  ,
}
where $\beta_{n}(\delta):= \eta\log\Big(\frac{\log(n)\log(\eta n)}{\delta \log^2(\eta)}\Big)$, with $\eta>1$ being an arbitrary parameter.
\end{lemma}

The next lemma presents a time-uniform concentration for i.i.d.~random variables with bounded support $[0,1]$:

\begin{lemma}
\label{lem:bounded_peeling}
 Let $Z = (Z_t)_{t\in \NN}$ be a sequence of i.i.d.~random  variables bounded in $[0,1]$, with mean $\mu$. Then, for all $\delta\in(0,1)$, it holds 
\als{
&\PP\bigg[\exists n\in \NN, \,\, \mu - \frac{1}{n}\sum_{t=1}^{n}Z_t \geq \sqrt{\frac{\beta_n(\delta)}{2n}} \bigg] \le \delta \, ,\\  
&\PP\bigg[\exists n\in \NN, \,\, \mu - \frac{1}{n}\sum_{t=1}^{n}Z_t \leq -\sqrt{\frac{\beta_n(\delta)}{2n}} \bigg] \le \delta\, ,
}
where $\beta_{n}(\delta):= \eta\log\Big(\frac{\log(n)\log(\eta n)}{\delta \log^2(\eta)}\Big)$, with $\eta>1$ being an arbitrary parameter.
\end{lemma}
% \sqrt{\frac{1+\eta}{2n}\log\left(\frac{\log(n)\log(n(1+\eta))}{\delta \log^2(1+\eta)}\right)

%\subsection{Proof of Lemma \ref{lem:CI_has_trueMDP}}
%\label{sec:proof_CI}
Both Lemma \ref{lem:Bernstein_peeling} and Lemma \ref{lem:bounded_peeling} are derived from Lemma~2.4 in \citep{maillard2019mathematics}. 



We also present the following lemma implying that the set of MDPs $\cM_{t,\delta}$ contains the true MDP by high probability:

\begin{lemma}\label{lem:CI_has_trueMDP}
For any FMDP with rewards in $\cR^{\text{fac}}_{\cX,[0,1]}(\cG_r)$, and transition function in $\cP^{\text{fac}}_{\cX,\cS}(\cG_p)$, for all $\delta\in(0,1)$, it holds
\als{
&\Pr\bigg(\exists t\in\Nat, x\in \cX, \quad  \mu(x) \notin \cC^r_{t,\delta}(x)
	\,\,\text{ or } \,\,P(\cdot|x) \notin \cC^p_{t,\delta}(x)\bigg)\leq 2\delta\,.
}	
In particular, for all $T\in \NN$:
\als{
\PP\big(\exists t\in \NN: M\notin \cM_{t,\delta}\big) \le 2\delta\, .
}	
\end{lemma}

\bp
First note that for any $i\in [\ell]$ and $x\in \cX[Z_i^r]$, by \citep[Theorem~10]{maurer2009empirical}:
$
\PP\big(\exists t\in \NN: \mu_i(x) \notin c_{t,\delta,i}(x)\big) \leq \delta. %\frac{\delta}{\ell|\cX[Z_i^r]|}.
$
Using union bounds and recalling that $\delta_i=\delta(\ell|\cX[Z_i^r]|)^{-1}$, it then follows that
\als{
\Pr\big(\exists t\in\Nat, x\in \cX, \quad  \mu(x) \notin \cC^r_{t,\delta}(x)\big)  &\leq \Pr\big(\exists i\in [\ell], x\in \cX[Z_i^r], \quad \mu_i(x) \notin c_{t,\delta_i,i}(x)\big) \\
&\leq \sum_{i\in [\ell]}\sum_{x\in \cX[Z_i^r]} \PP\big(\exists t\in \NN: \mu_i(x) \notin c_{t,\delta_i,i}(x)\big) \\
&\leq \sum_{i\in [\ell]}\sum_{x\in \cX[Z_i^r]}  \frac{\delta}{\ell|\cX[Z_i^r]|} = \delta.
}	

Now we consider the case of transition function. 
For any $i\in [m]$, $x\in \cX[Z_i^m]$, and $y\in \cS_i$, Lemma \ref{lem:Bernstein_peeling} implies:
$$
\PP\big(\exists t\in \NN: P_i(y|x) \notin C_{t,\delta,i}(x,y)\big) \leq \frac{\delta}{mS_i|\cX[Z_i^p]|}
$$
Using union bounds gives
\als{
\Pr\big(\exists t\in\Nat, x\in \cX, \,  P(\cdot|x) \notin \cC^p_{t,\delta}(x)\big)  &\leq \Pr\big(\exists i\in [m], x\in \cX[Z_i^p], y\in \cS_i, \, P_i(y|x) \notin C_{t,\delta,i}(x,y)\big) \\
&\leq \sum_{i\in [m]}\sum_{x\in \cX[Z_i^p]}\sum_{y\in \cS_i} \PP\big(\exists t\in \NN: P_i(y|x) \notin C_{t,\delta,i}(x,y)\big) \leq \delta.
}	
Putting together and taking a union bound complete the proof. 
\ep


\section{Regret Analysis: Generic Structures (Theorem \ref{thm:regret_Alg1})}
\label{app:regret_proof_generic}

In this section, we prove Theorem \ref{thm:regret_Alg1}. Before presenting the proof, we collect some necessary lemmas. 


\subsection{Proof of Theorem \ref{thm:regret_Alg1}}

%\noindent{\it Proof (of Theorem \ref{thm:regret_Alg1}).}
Our proof follows similar lines as in the proof of \citep[Theorem~2]{jaksch2010near}. Let $\delta\in (0,1)$. To simplify notations, let us define the short-hand $J_k:=J_{t_k}$ for various random variables that are fixed within a given episode $k$ and omit their dependence on $\delta$ (for example, $\cM_{k}:=\cM_{t_k,\delta}$). Denote by $K(T)$ the number of episodes initiated by the algorithm up to time $T$. {\color{black}Given a pair $x=(s,a)$, let $N_t(x)$ denote the number of times $x$ is selected by the algorithm up to time $t$. Furthermore, let $n_k(x)$ denote the number of times $x$ is sampled in a given episode $k$.}

%$\text{N}(t, x; Z) := \max(\sum_{t'=1}^{t-1} \indic{x_{t'}[Z] = x}, 1)$ denote the number of visits to $x$ up to time $t$. Let us consider time $t\ge 1$ and recall that $x_t = (s_t, a_t)$. 
%For $i\!\in\! [m]$ we define the shorthand notation $N^p_{i,t}(x):= \text{N}(t, x; Z^p_i)$. Likewise, for $i\!\in\! [\ell]$ we define $N^r_{i,t}(x):= \text{N}(t, x; Z^r_i)$. We then introduce the following empirical estimates: Given $i\!\in\! [m], x\!\in\! \cX[Z^p_i]$, we let $\widehat P_{i,t}(\cdot|x)$  be the empirical distribution built using $N^p_{i,t}(x)$ i.i.d.~samples from $P_{i}(\cdot|x)$. Similarly,  given $i\in [\ell]$ and $x\in \cX[Z^r_i]$, we define $\widehat \mu_{i,t}(x)$ as the empirical estimate of $R_i(x)$ built using $N^r_{i,t}(x)$ i.i.d.~samples from $R_i(x)$. More precisely, 


By applying Lemma \ref{lem:bounded_peeling} and noting that $r_t[i]\in [0,1]$, we deduce that
% For Laplace:
%\als{
%\kR(T)&= \sum_{t=1}^T g^\star- \sum_{t=1}^T \sum_{i=1}^\ell r_t[i] \leq \sum_{x\in \cX} N_{T}(x)\big(g_\star - \sum_{i=1}^\ell \mu_i(x[Z_i^r])\big) + \sqrt{ \tfrac{1}{2}(T+1) \log( \sqrt{T+1}/\delta)}\, ,
%}
\als{
\kR(T)&= \sum_{t=1}^T g^\star- \sum_{t=1}^T \frac{1}{\ell}\sum_{i=1}^\ell r_t[i] \leq \sum_{x\in \cX} N_{T}(x)\Big(g^\star -  \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big) + \sqrt{T\beta_T(\delta)/2}\, ,
}
with probability at least $1-\delta$. We have
\als{
\sum_{x} N_{T}(x)\Big(g^\star - \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x)\Big) &= \sum_{k=1}^{K(T)}  \sum_{x}  \sum_{t=t_k}^{t_{k+1}-1}\indic{x_t=x} \Big(g^\star - \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big)\\
&=
\sum_{k=1}^{K(T)} \sum_{x} n_k(x) \Big(g^\star - \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big)\,.
}
Introducing $\Delta_k := \sum_{x\in \cX} n_k(x) \Big(g^\star - \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big)$ for $1\leq k\leq K(T)$, we get
\als{
\kR(T) \le \sum_{k=1}^{K(T)} \Delta_k + \sqrt{T\beta_T(\delta)/2} \,, % \sqrt{ \tfrac{1}{2}(T+1) \log( \sqrt{T+1}/\delta)}\, ,
}
with probability at least $1-\delta$. A given episode $k$ is called \emph{good} if $M \in \cM_{k}$ (that is, the set of plausible MDPs contains the true model), and \emph{bad} otherwise. By Lemma \ref{lem:CI_has_trueMDP}, for all $T$, and for all episodes $k=1,\ldots,K(T)$, the set $\cM_{k}$ contains the true MDP with probability higher than $1-2\delta$. As a consequence, with probability at least $1-2\delta$, $
\sum_{k=1}^{K(T)}\Delta_k\indic{M \notin \cM_{k}} = 0.
$

To upper bound regret in good episodes, we closely follow \citep{jaksch2010near} and decompose the regret to control the transition and reward functions. Consider a good episode $k$ (hence, $M \in \cM_{k}$). By choosing $\pi^+_{k}$ and $\widetilde M_{k}$, we get that
$$
g_k := g_{\pi^+_{k}}^{\widetilde M_{k}} \geq g^\star - \frac{1}{\sqrt{t_k}}\, ,
$$
so that with probability greater than $1-\delta$,
\begin{align}
\Delta_k  &\leq \sum_{x\in \cX} n_k(x)
\Big(g_k - \frac{1}{\ell}\sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big) + \sum_{x\in \cX} \frac{n_k(x)}{\sqrt{t_k}} 
\, .
\label{eq:delta_init}
\end{align}
Using the same argument as in the proof of \citep[Theorem~2]{jaksch2010near}, the value function $u_k^{(l)}$ computed by \EVI\ at iteration $l$ satisfies: $\max_{s} u_k^{(l)}(s) - \min_{s} u_k^{(l)}(s) \leq D$. The convergence criterion of \EVI\ implies
\begin{equation}
|u_k^{(l+1)}(s) - u_k^{(l)}(s) - g_k| \leq \frac{1}{\sqrt{t_k}}\,, \qquad  \forall s \in \cS\, .
\label{eq:puterman_convergence}
\end{equation}
Using the Bellman operator on the optimistic MDP:
\als{
u_k^{(l+1)}(s) &= \frac{1}{\ell}\sum_{i=1}^\ell \widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i^r]) + \sum_{s'} \widetilde P_k(s'|s,\pi^+_{k}(s)) u_k^{(l)}(s') \\
&= \frac{1}{\ell}\sum_{i=1}^\ell \widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i^r]) + \sum_{s'} \widetilde P_{k}(s'|s,\pi^+_{k}(s)) u_k^{(l)}(s')\,.
}
Substituting this into (\ref{eq:puterman_convergence}) gives
\begin{equation*}
\Big|\Big( g_k - \frac{1}{\ell}\sum_{i=1}^\ell \widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i^r]) \Big) - \Big(\sum_{s'} \widetilde P_{k}(s'|s,\pi^+_{k}(s))u_k^{(l)}(s') - u_k^{(l)}(s)\Big)\Big|
\leq \frac{1}{\sqrt{t_k}}\, , \qquad \forall s\in \cS\, .
\end{equation*}
Defining
${\bf g}_k = g_k \mathbf 1$, $\widetilde{\boldsymbol{\mu}}_{k} := \big(\widetilde\mu_{k}(s,\pi^+_k(s))\big)_s$, $\widetilde{\mathbf{P}}_k := \big(\widetilde P_{k}\big(s'|s,\pi^+_k(s)\big)\big)_{s, s'}$ and $n_{k} := \big(n_k\big(s,\pi^+_k(s)\big)\big)_s$, we can rewrite the above inequality as:
\begin{equation*}
\Big|{\bf g}_k - \frac{1}{\ell}\widetilde{\boldsymbol{\mu}}_{k} - (\widetilde{\mathbf{P}}_k - \mathbf{I}) u_k^{(l)} \Big|
\leq \frac{1}{\sqrt{t_k}}\mathbf 1\,.
\end{equation*}
Combining this with (\ref{eq:delta_init}) yields
\begin{align}
\Delta_k&\leq \sum_{x} n_k(x) \Big(g_k-\frac{1}{\ell} \sum_{i=1}^\ell \mu_i(x[Z_i^r])\Big) +  \sum_{x} \frac{n_k(x)}{\sqrt{t_k}} \nonumber\\
&= \sum_{x} n_k(x) \Big( g_k - \frac{1}{\ell}\sum_{i=1}^\ell  \widetilde\mu_{i,k}(x[Z_i^r]) \Big) + \frac{1}{\ell}\sum_{x} n_k(x) \sum_{i=1}^\ell\big( \widetilde\mu_{i,k}(x[Z_i^r]) - \mu_{i}(x[Z_i^r]) \big) +  \sum_{x} \frac{n_k(x)}{\sqrt{t_k}} \nonumber\\
&\leq n_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) u_k^{(l)} + \frac{1}{\ell}\sum_{x} n_k(x) \sum_{i=1}^\ell \big(\widetilde\mu_{i,k}(x[Z_i^r]) - \mu_i(x[Z_i^r]) \big) +  2\sum_{x} \frac{n_k(x)}{\sqrt{t_k}} \, .\nonumber
\end{align}
Similarly to \citep{jaksch2010near}, we define $w_k(s) := u_k^{(l)}(s) - \tfrac{1}{2}(\min_s u_k^{(l)}(s) + \max_s u_k^{(l)}(s))$ for all $s\in \cS$. Then, in view of the fact that $\widetilde{\mathbf{P}}_k$ is row-stochastic, we obtain
\begin{align}
\Delta_k&\leq n_{k} (\widetilde{\mathbf{P}}_k - \mathbf{I} ) w_k + \frac{1}{\ell}\sum_{x} n_k(x) \sum_{i=1}^\ell \big(\widetilde \mu_{i,k}(x[Z_i^r]) - \mu_i(x[Z_i^r]) \big) +  2\sum_{x} \frac{n_k(x)}{\sqrt{t_k}}\, .
\end{align}
The second term in the right-hand side can be upper bounded as follows: $M \in \cM_{k}$ implies that %for $x=(s,a)$
\als{
\sum_{i=1}^\ell \big(\widetilde \mu_{i,k}(x[Z_i^r]) - \mu_{i}(x[Z_i^r])\big) &\leq 2\sum_{i=1}^\ell \sqrt{\frac{2\widehat\sigma_{i,k}^2(x[Z_i^r])}{N^r_{i,t}(x[Z_i^r])}\beta_{N^r_{i,k}(x[Z_i^r])}\Big(\frac{\delta}{\ell|\cX[Z_i^r]|}\Big)} + 2\sum_{i=1}^\ell\frac{7}{3N^r_{i,t}(x[Z_i^r])}\beta_{N^r_{i,t}(x[Z_i^r])}\Big(\frac{\delta}{\ell|\cX[Z_i^r]|}\Big)\\
&\leq \sum_{i=1}^\ell \sqrt{\frac{2}{N^r_{i,k}(x[Z_i^r])}\beta_{T}\Big(\frac{\delta}{\ell|\cX[Z_i^r]|}\Big)} + \frac{14}{3}\sum_{i=1}^\ell\frac{1}{N^r_{i,k}(x[Z_i^r])}\beta_{T}\Big(\frac{\delta}{\ell|\cX[Z_i^r]|}\Big)
   \, ,
}
where we have used $\widehat\sigma_{i,k}^2(x[Z_i^r])\le \tfrac{1}{4}$ and $1\leq N^r_{i,k}(x[Z_i^r]) \leq T$ in the last inequality. Furthermore, since  $t_k\ge \max_{i\in [\ell]} N^r_{i,k}(x[Z_i^r])$, we have
\als{
\sum_{x}  \frac{n_k(x)}{\sqrt{t_k}} &\le \sum_{x}  \sum_{i=1}^\ell \frac{n_k(x)}{\sqrt{N^r_{i,k}(x[Z_i^r])}}\, .
}
Putting together, and denoting $\beta_{T,i}:= \beta_{T}\Big(\frac{\delta}{\ell|\cX[Z_i^r]|}\Big)$, we obtain
%\begin{align}
%\Delta_k
%&\leq n_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 
%2\sum_{i=1}^\ell  \Big(\sqrt{\log\Big(3 |\cX[Z_i^r]|\sqrt{T\!+\!1}/\delta\Big)} + 1\Big) \sum_{x\in \cX}\frac{n_k(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} \sk
%&\leq n_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 
%2\sum_{i=1}^\ell \Big(\sqrt{\log\Big(3 |\cX[Z_i^r]|\sqrt{T\!+\!1}/\delta\Big)} + 1\Big) \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} \, ,
%\label{eq:main_delta_minmk}\end{align}
\begin{align}
\Delta_k
&\leq n_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 
\frac{\sqrt{2}}{\ell}\sum_{i=1}^\ell  \sqrt{\beta_{T,i}} \sum_{x\in \cX}\frac{n_k(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} + \frac{14}{3\ell}\sum_{i=1}^\ell  \beta_{T,i} \sum_{x\in \cX}\frac{n_k(x)}{N_{i,k}^r(x[Z_i^r])} \sk
&\leq n_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k + 
\frac{\sqrt{2}}{\ell}\sum_{i=1}^\ell  \sqrt{\beta_{T,i}}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} + \frac{14}{3\ell}\sum_{i=1}^\ell  \beta_{T,i}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{N_{i,k}^r(x[Z_i^r])} \, ,
\label{eq:main_delta_minmk}\end{align}
where the last inequality follows from Lemma \ref{lem:factored_count}, stated and proven in Section \ref{sec:supp_lemmas}.

In what follows, we derive an upper bound on $n_{k} (\widetilde{\mathbf{P}}_k-\mathbf{I})w_k$. Similarly to \citep{jaksch2010near}, we consider the following decomposition:
\als{
n_k(\widetilde{\mathbf{P}}_k - \mathbf{I}) w_k = \underbrace{n_k (\widetilde{\mathbf{P}}_k - \mathbf{P}_k) w_k}_{L_1(k)} + \underbrace{n_k (\mathbf{P}_k-\mathbf{I})w_k}_{L_2(k)} \, .
}

The following lemmas provide upper bounds on $L_1(k)$ and $L_2(k)$:

\begin{lemma}\label{lem:L_1_k}
Consider a good episode $k$. Then,
\als{
L_1(k) &\leq 3\sum_{i=1}^m \sqrt{\beta'_{T,i}}\sum_{x=(s,a)\in \cX[Z_i^p]} \nu^p_k(x)  D_{i,s}\sqrt{\frac{K_{i,x} - 1}{N^p_{i,k}(x)}}
 + 5\sum_{i=1}^m  DS_i\beta'_{T,i}\sum_{x\in \cX[Z_i^p]}  \frac{\nu_{i,k}^p(x)}{N^p_{i,k}(x)} \, ,
}
where $\beta'_{T,i}:= \beta_T\big(\tfrac{\delta}{mS_i|\cX[Z_i^p]|}\big)$. 
\end{lemma}

\begin{lemma}\label{lem:L_2_k}
For all $T$, it holds with probability at least $1-\delta$,
\als{
\sum_{k=1}^{K(T)} L_2(k) \bI\{M \in \cM_{k}\} \leq \max_{i,s\in \cS[Z_i^p]} D_{i,s} \max_{(s,a)\in \cX} \sum_{i=1}^m K_{i,s[Z_i^p],a[Z_i^p]} D_{i,s} \sqrt{2T \beta_T(\delta)} + D K(T) \, .
%\label{eq:trans_prob_second_overall_minmk}
}
\end{lemma}

Applying Lemmas \ref{lem:L_1_k} and \ref{lem:L_2_k}, and summing over all good episodes, we obtain the following bound that holds
 with probability higher than $1-2\delta$, uniformly over all $T\in\Nat$:
\begin{align}
\sum_{k=1}^{K(T)} \Delta_k &\bI\{M \in \cM_{k}\} \leq
\sum_{k=1}^{K(T)} L_1(k) + \sum_{k=1}^{K(T)} L_2(k) + %2\sum_{i=1}^\ell  \beta'_T\sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}}
\frac{\sqrt{2}}{\ell}\sum_{i=1}^\ell  \sqrt{\beta_{T,i}}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} \\
&+ \frac{14}{3\ell}\sum_{i=1}^\ell  \beta_{T,i}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{N_{i,k}^r(x[Z_i^r])} 
 \nonumber \\
&\leq 3\sum_{i=1}^m \sqrt{\beta'_{T,i}}\sum_{x=(s,a)\in \cX[Z_i^p]}    D_{i,s}\sqrt{K_{i,x} - 1}\frac{\nu^p_{i,k}(x)}{\sqrt{N^p_{i,k}(x)}}
 + 5 \sum_{i=1}^m DS_i\beta'_{T,i}\sum_{x\in \cX[Z_i^p]}  \frac{\nu_{i,k}^p(x)}{N^p_{i,k}(x)} \sk
 &+ \frac{\sqrt{2}}{\ell}\sum_{i=1}^\ell  \sqrt{\beta_{T,i}}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} + \frac{14}{3\ell}\sum_{i=1}^\ell  \beta_{T,i}  \sum_{x\in \cX[Z_i^r]} \frac{\nu_{i,k}^r(x)}{N_{i,k}^r(x[Z_i^r])} \sk
 &+ 2\sum_{i=1}^\ell \sum_{x\in \cX[Z_i^r]} \beta_T' \frac{n_k(x)}{\sqrt{N_{i,k}^r(x[Z_i^r])}} +  \max_{i,s\in\cS[Z_i^p]} D_{i,s} \sqrt{2T \beta_T(\delta)} + D K(T) \, .
\label{eq:trans_prob_intermed_minmk}
\end{align}

To simplify the above bound, we provide the following lemma:
\begin{lemma}\label{lem:N_k_sequenence_sums}
	Consider a set $\cX'$, and for $x\in \cX'$, let $\nu_k(x)$ (resp.~$N_k(x)$) denote the number of times $x$ is oberserved in episode $k$ (resp.~before episode $k$ starts). We have:
\als{
(i)& \qquad \sum_{x\in \cX'} \sum_{k=1}^{K(T)} \frac{\nu_k(x)\alpha(x)}{\sqrt{N_{k}(x)}}  \leq
	\big( \sqrt{2} + 1 \big) \sqrt{T\sum_{x\in \cX'}\alpha(x)}\, . \\
(ii)& \qquad \sum_{x\in \cX'} \sum_{k=1}^{K(T)} \frac{\nu_k(x)}{N_{k}(x)}  \leq
 2|\cX'|\log\big(\tfrac{T}{|\cX'|}\big) + |\cX'|\, .
}
\end{lemma}

Moreover, following the same lines in the proof of \citep[Proposition]{jaksch2010near} (i.e., upper bounding the number of episodes), one has that the number of episodes $K(T)$ is no more than 
\als{
\sum_{i=1}^m |\cX[Z_i^p]|\log_2\big(\tfrac{T}{|\cX[Z_i^p]|}\big) + \sum_{i=1}^\ell |\cX[Z_i^r]|\log_2\big(\tfrac{T}{|\cX[Z_i^r]|}\big)\, .
}

%\begin{lemma}[{\cite[Lemma~19]{jaksch2010near}}]\label{lem:sequence}
%	For any sequence of numbers $z_1, z_2, \dots, z_n$ with $0 \leq z_k \leq Z_{k-1} := \max\{1, \sum_{i=1}^{k-1}z_i\}$,
%	$$
%	\sum_{k=1}^n 	\frac{z_k}{\sqrt{Z_{k-1}}} 	\leq 	\big(\sqrt{2} + 1\big) 	\sqrt{Z_n}\, .
%	$$
%\end{lemma}
%\begin{lemma}[{\cite[Lemma~24]{talebi2018variance}}]
%\label{lem:seq_harmonic}
%Consider a sequence $(z_k)_{1\leq k\leq n}$ with $0\leq z_k \leq Z_{k-1}:=\max\bigl\{1,\sum_{i=1}^{k-1} z_i\big\}$ for $k\geq  1$ and $Z_0= z_1$. Then,
%\begin{align*}
%\sum_{k=1}^n \frac{z_k}{Z_{k-1}} \leq 2\log(Z_n) + 1\, .
%\end{align*}
%\end{lemma}
%\begin{lemma}
%\label{lem:seq_2over3}
%Consider a sequence $(z_k)_{1\leq k\leq n}$ with $0\leq z_k \leq Z_{k-1}:=\max\bigl\{1,\sum_{i=1}^{k-1} z_i\big\}$ for $k\geq  1$ and $Z_0= z_1$. Then, for some universal constant $C$,
%\begin{align*}
%\sum_{k=1}^n \frac{z_k}{Z_{k-1}^{2/3}} \leq C Z_n^{1/3}\, .
%\end{align*}
%\end{lemma}

% Applying Lemmas \ref{lem:sequence}-\ref{lem:seq_2over3}, and using Jensen's inequality yield:

%Applying Lemma \ref{lem:sequence_sums} and using Jensen's inequality yield:
%\als{
%&\sum_{s,a} \sum_{k=1}^{K(T)} \frac{\nu_k(s,a)}{\sqrt{N_{k}(s,a)^+}}  \leq
%\sum_{s,a} \big(\sqrt{2} + 1\big) \sqrt{N_{K(T)}(s,a)} \le	\big( \sqrt{2} + 1 \big) \sqrt{SAT}\, ,\sk
%&\sum_{s,a} \sum_{k=1}^{K(T)} \frac{\nu_k(s,a)}{\sqrt{N_{k}(s,a)^+}}D_sL_{s,a}  \leq
%\sum_{s,a} \big(\sqrt{2} + 1\big) \sqrt{N_{K(T)}(s,a)} \le	\big( \sqrt{2} + 1 \big) ....\, ,\sk
%&\sum_{s,a} \sum_{k=1}^{K(T)} \frac{\nu_k(s,a)}{N_{k}(s,a)^+}  \leq
%2\sum_{s,a} \log(N_{K(T)}(s,a)) + SA \leq 2SA\log\big(\tfrac{T}{SA}\big) + SA\, ,\sk
%&\sum_{s,a} \sum_{k=1}^{K(T)} \frac{\nu_k(s,a)}{(N_{k}(s,a)^+)^{2/3}}  \leq
%C \sum_{s,a} N_{K(T)}(s,a)^{1/3} \leq C(SA)^{2/3}T^{1/3}\, .
%}

Putting everything together, it holds that with probability at least $1-5\delta$,
\als{
\kR(T) &\leq 
8 \sum_{i=1}^m \sqrt{\beta_{T,i}'\sum_{x=(s,a)\in \cX[Z_i^p]} D^2_{i,s} (K_{i,x} - 1) T} + \frac{4}{\ell}\sum_{i=1}^\ell  \sqrt{\beta_{T,i}|\cX[X_i^r]|T} \\
& \frac{6}{\ell}\sum_{i=1}^\ell \beta_{T,i}|\cX[Z_i^r]| \log\big(\tfrac{T}{|\cX[Z_i^r]|}\big) + 10\sum_{i=1}^m D S_i\beta_{T,i}'|\cX[Z_i^p]| \log\big(\tfrac{T}{|\cX[Z_i^p]|}\big) \sk
 &+  \big(\max_{i,s\in\cS[Z_i^p]} D_{i,s}\sqrt{2} + \sqrt{\tfrac{1}{2}}\big) \sqrt{T\beta_T(\delta)} + D\Big( \sum_{i=1}^m |\cX[Z_i^p]|\log_2\big(\tfrac{T}{|\cX[Z_i^p]|}\big) + \sum_{i=1}^\ell |\cX[Z_i^r]|\log_2\big(\tfrac{T}{|\cX[Z_i^r]|}\big)\Big) \, .
}
Noting that $\beta_T,\beta_{T,i},\beta'_{T,i} = \cO(\log(\log(T)))$ gives the desired result and completes the proof. 
%\als{
%5\sqrt{\sum\nolimits_{s,a} D_s^2 L_{s,a}} + 4\sqrt{SA} \leq 10\sqrt{SA \!+\! \sum\nolimits_{s,a} D_s^2L_{s,a} } \leq 10\sqrt{2\sum\nolimits_{s,a} \big(D_s^2L_{s,a}\big)^+}\, ,
%}
\ep

%\begin{myproof}{(of Lemma \ref{lem:SqrtVar_pqBern})}


\subsection{Proof of Technical Lemmas}

\subsubsection{Proof of Lemma \ref{lem:L_1_k}}
%\noindent{\it Proof of Lemma \ref{lem:L_1_k}.} 
Recall that %To derive an upper bound on $L_1(k)$, first notice that
\als{
L_1(k)  &= \sum_{s\in \cS}n_k(s,\pi^+_k(s)) \sum_{y\in \cS} \big(\widetilde P_k -  P_k\big)\big(y|s,\pi^+_k(s)\big) w_k(y)\\
&\leq \sum_{s\in \cS}n_k(s,\pi^+_k(s)) \sum_{y\in \cS} \big|\big(\widetilde P_k -  P_k\big)\big(y|s,\pi^+_k(s)\big)\big| \big|w_k(y)\big|\, . 
}

Fix $s\in \cS$, and introduce $x^k:= (s,\pi^+_k(s))$. We have%Using Lemma \ref{lem:factored_deviation} with {\color{red}$...$} we have 
\als{
\sum_{y\in \cS} \big(\widetilde P_k -  P_k)\big(y|s,\pi^+_k(s)\big) w_k(y) &\leq \underbrace{\sum_{y\in \cS} \big|\big(\widehat P_k - P_k\big)\big(y|x^k\big)\big| \big|w_k(y)\big|}_{F_1} + \underbrace{\sum_{y\in \cS} \big|\big(\widetilde P_k - \widehat P_k\big)\big(y|x^k\big)\big| \big|w_k(y)\big|}_{F_2}\, .
}

To upper bound $F_1$, let us define
$$
%H_k(x^k) := \max_{y\in\otimes_{i=1}^m \supp(P_{i}(\cdot|x^k[Z^p_i])} |w(y)|\, ,
H_k(x^k) := \max_{y\in\otimes_{i=1}^m \cK_{i,x^k[Z^p_i]}} |w(y)|\, , 
$$
where we recall that $\cK_{i,x}:=\supp(P_i(\cdot|x))$. Now an application of Lemma \ref{lem:factored_deviation} gives:
\als{
F_1 &\leq  H_k(x^k)\sum_{i=1}^m \sqrt{\frac{2\beta_T}{N^p_{i,k}(x^k[Z^p_i])}} \sum_{y[i]\in \cS_i} \sqrt{P_{i}(1-P_i)(y[i]|x^k[Z^p_i])}  + \sum_{i=1}^m \frac{ DS_i\beta_{T,i}'}{6N^p_{i,k}(x^k[Z^p_i])}\, .
}
where we used that $\max_{y\in \cS} |w(y)|\leq \tfrac{D}{2}$ (following a similar argument as in \citep{jaksch2010near}), and defined the short-hand $\beta_{T,i}':=\beta_T(\tfrac{\delta}{mS_i|\cX[Z_i^p]|})$. 
 
By Cauchy-Schwarz, we get
%\als{
%\sum_{y[i]\in \cS_i} &\sqrt{P_i(1-P_i)(y|x^k[Z^p_i])} =  \sum_{y[i]\in \supp(P_i(\cdot|x^k[Z^p_i])} \sqrt{P_i(1-P_i)(y[i]|x^k[Z^p_i])} \\
%&\leq  \sqrt{\sum_{y[i]\in \supp(P_i(\cdot|x^k[Z^p_i])} P_i(y[i]|x^k[Z_i^p])} \sqrt{\sum_{y[i]\in \supp(P_i(\cdot|x^k[Z^p_i])} (1-P_i)(y[i]|x^k[Z_i])} \\
%&\leq  \sqrt{|\supp(P_i(\cdot|x^k[Z^p_i])| -1} \, ,
%}
\als{
\sum_{y[i]\in \cS_i} &\sqrt{P_i(1-P_i)(y|x^k[Z^p_i])} =  \sum_{y[i]\in \cK_{i,x^k[Z^p_i]}} \sqrt{P_i(1-P_i)(y[i]|x^k[Z^p_i])} \\
&\leq  \sqrt{  \sum_{y[i]\in \cK_{i,x^k[Z^p_i]}  } P_i(y[i]|x^k[Z_i^p])} \sqrt{\sum_{y[i]\in \cK_{i,x^k[Z^p_i]}  } (1-P_i)(y[i]|x^k[Z_i])} \\
&\leq  \sqrt{K_{i,x^k[Z^p_i]} -1} \, ,
}
so that
\als{
F_1 &\leq H_k(x^k)\sum_{i=1}^m \sqrt{\frac{2\beta_{T,i}'}{N^p_{i,k}(x^k[Z^p_i])}} \sqrt{K_{i,x^k[Z^p_i]} -1}  + \sum_{i=1}^m \frac{DS_i\beta_{T,i}'}{6N^p_{i,k}(x^k[Z^p_i])} \, .
}

To upper bound $F_2$, we will need the following lemma:

\begin{lemma}
	\label{lem:SqrtVar_pqBern}
	Consider $x$ and $y$ satisfying $|x - y| \leq \sqrt{2y(1-y)\zeta} + \zeta/3$. Then,
\begin{align*}
\sqrt{y(1 - y)} &\leq \sqrt{x(1- x)} + 2.4\sqrt{\zeta} \, .
	\end{align*}
\end{lemma}

Applying this lemma twice, we have that for any $y$ and $x$, if $|\widetilde P_{i,k} - \widehat P_{i,k}|(y|x) \leq \sqrt{2\widetilde P_{i,k}(1-\widetilde P_{i,k})(y|x)\zeta} + \zeta'/3$, where $\zeta,\zeta'$ come from the definition of $C_{t,\delta,i}(x,y)$, then
\als{
|\widetilde P_{i,k} - \widehat P_{i,k}|(y|x) \leq \sqrt{2P_i(1-P_i)(y|x)\zeta} + 4\zeta'. 
}
Hence, an application of Lemma  \ref{lem:factored_deviation} gives 
\als{
F_2 &\leq H_k(x^k)\sum_{i=1}^m \sqrt{\frac{2\beta_{T,i}'}{N^p_{i,k}(x^k[Z^p_i])}} \sqrt{K_{i,x^k[Z^p_i]} -1}  + 4 \sum_{i=1}^m \frac{DS_i\beta_{T,i}'}{N^p_{i,k}(x^k[Z^p_i])} \, .
}

Putting together, we get
\als{
L_1(k) &\leq 3\sum_{x\in \cX} n_k(x)H_k(x)\sum_{i=1}^m \sqrt{\frac{\beta_{T,i}'}{N^p_{i,k}(x[Z^p_i])}} \sqrt{K_{i,x[Z^p_i]} -1} 
 + 5 \sum_{x\in \cX} \nu^p_k(x) \sum_{i=1}^m \frac{DS_i\beta_{T,i}'}{2N^p_{i,k}(x[Z^p_i])}  \, .
}

To control the right-hand side, we further show that given $x\in \cX$,
$$
H_k(x) \leq \max_{u=(s,a): u[Z_i^p]=x}\max_{y\in \cL_s} |w(y)| \leq D_{i,s[Z_i^p]}, \quad \forall i\in [m].
$$
where $\cL_{s} := \otimes_{i=1}^m(\cup_{a\in \cA[Z^p_i]} \cK_{i, s[Z_i^p], a})$


The first inequality holds by definition of $H_k$. To verify the second claim,  we note that similarly to \citep{jaksch2010near}, we can combine all MDPs in $\cM_k$ to form a single MDP $\widetilde\cM_k$ with continuous action space $\cA'$. In this extended MDP, in each state $s\in \cS$, and for each $a\in \cA$, there is an action in $\cA'$ with mean $\tilde\mu(s,a)$ and transition $\widetilde P(\cdot|s,a)$ satisfying the definition of the set of plausible MDPs. Similarly to the arguments in \citep{jaksch2010near}, we recall that $u^{(l)}_k(s)$ amounts to the total expected $l$-step reward of an optimal non-stationary $l$-step policy starting in state $s$ on the MDP $\widetilde\cM_k$ with extended action set. Recall that we are in a case where $M\in \cM_k$. This implies that the local diameter of factor $i$ and state $s$ of this extended MDP is at most $D_{i,s[Z_i^p]}$, since the actions of the true MDP are contained in the continuous action set of the extended MDP $\widetilde\cM_k$. 
Let 
\als{
\cB_i:= \Big\{y\in \cS: y[i]\in \cup_{a'\in \cA[Z_i^p]} \cK_{i,s[Z_i^p], a'}\, \hbox{ and }  \, y[j]\in \cS_j, i\neq j\Big\}.
}
Now, if there were states $s_1,s_2\in \cB_i$ with $u^{(l)}_k(s_1) - u^{(l)}_k(s_2) >  D_{i,s[Z_i^p]}$, then an improved value
for $u^{(l)}_k(s_1)$ could be achieved by the following non-stationary policy: First follow a policy which moves from $s_1$ to $s_2$ most quickly, which takes at most $D_{i,s[Z_i^p]}$ steps on average. Then follow the optimal $l$-step policy for $s_2$. We thus have $u^{(l)}_k(s_1) \geq u^{(l)}_k(s_2)- D_{i,s[Z_i^p]}$, since at most $D_{i,s[Z_i^p]}$ rewards of the policy for $s_2$ are missed. This is a contradiction, and so the claim follows. %Using a similar argument yields: $\max_{x\in \supp(p(\cdot|s,a))}|w_k(x)| \leq \tfrac{D_s}{2}$.
	
%\max_{s\in \cS: s[Z^p_i] = u} \max_{s_1,s_2\in \cL_{s}} \min_\pi \EE[T^\pi(s_1,s_2)]\, ,
%}
%where $\cL_{s} := \otimes_{i=1}^m(\cup_{a\in \cA[Z^p_i]} \cK_{i, s[Z_i^p], a})$,	
	
		
Hence,
\als{
L_1(k) &\leq 3\sum_{i=1}^m \sum_{x\in \cX} n_k(x) D_{i,s[Z_i^p]} \sqrt{\frac{\beta_{T,i}'}{N^p_{i,k}(x[Z^p_i])}} \sqrt{(K_{i,x[Z^p_i]} - 1) }
 + 5 \sum_{i=1}^m \sum_{x\in \cX}  n_k(x)\frac{DS_i\beta_{T,i}'}{N^p_{i,k}(x[Z^p_i])} \\
 &\leq 3\sum_{i=1}^m \sum_{x=(s,a)\in \cX[Z_i^p]} \nu^p_{i,k}(x)  D_{i,s[Z_i^p]}\sqrt{\frac{\beta_{T,i}' (K_{i,x} - 1)}{N^p_{i,k}(x)}}
 + 5 \sum_{i=1}^m DS_i\beta_{T,i}' \sum_{x\in \cX[Z_i^p]}  \frac{\nu_{i,k}^p(x)}{N^p_{i,k}(x)} 
 \, ,
}
where the last inequality follows from Lemma \ref{lem:factored_count}. 
%	Combininig the bounds on $F_1$ and $F_2$, and noting that 
%	\als{
%		\ell_{N_k(s,a)}\big(\tfrac{\delta}{3(1+S)SA}\big) \leq \ell_{N_k(s,a)}\big(\tfrac{\delta}{6S^2A}\big) \leq \ell_{T}\big(\tfrac{\delta}{6S^2A}\big)
%	}
%	complete the proof. 
\ep



\subsubsection{Proof of Lemma \ref{lem:L_2_k}}
%\noindent{\it Proof of Lemma \ref{lem:L_2_k}.}
The proof follows similar steps as in the proof of \citep[Theorem~2]{jaksch2010near}. Here, we collect all necessary arguments for completeness. Let us define the sequence $(X_t)_{t\geq 1}$ with $X_t := (P(\cdot|s_t,a_t) - \mathbf e_{s_{t+1}})w_{k(t)}\bI\{M \in \cM_{k(t)}\}$, for all $t$, where $k(t)$ denotes the episode containing step $t$. For any $k$ with $M \in \cM_{k}$, we have that:
	\als{
		L_2(k) &= \nu_k (\mathbf{P}_k-\mathbf{I})w_k  = \sum_{t=t_k}^{t_{k+1} -1} (P(\cdot|s_t,a_t) - \mathbf{e}_{s_t}) w_k \\
				&= \sum_{t=t_k}^{t_{k+1} -1} X_t + w_k(s_{t+1}) - w_k(s_t) \leq \sum_{t=t_k}^{t_{k+1} -1} X_t + D \, ,
	}
	so that $\sum_{k=1}^{K(T)} L_2(k) \leq \sum_{t=1}^T
	X_t +K(T)D$. 
	Observe that:
	\als{
	X_t &= (P(\cdot|s_t,a_t) - \mathbf e_{s_{t+1}})w_{k(t)}\bI\{M \in \cM_{k(t)}\} \\
	&= \sum_{y\in \cS}\Big( \prod_{i=1}^mP_i\big(y[i]|s_t[Z_i^p], a_t[Z_i^p]\big) - \bI\{s_t[1] = y[1], \ldots, s_t[m]=y[m]\} \Big)
	}	
	Noting that $|P_i\big(y[i]|s_t[Z_i^p], a_t[Z_i^p]\big) - \bI\{s_t[i]=y[i]\}|\le 2 \bI\{y[i]\in \mathrm{supp}(P_i(\cdot|s_t[Z_i^p], a_t[Z_i^p]))$, we can apply Lemma \ref{lem:factored_deviation} to obtain:
	\als{
	|X_t| &\le 2\max_{y\in \cL_{s_t,a_t}} |w_{k(t)}(y)| \sum_{i=1}^m \sum_{y\in \cS_i} \bI\{y[i]\in \mathrm{supp}(P_i(\cdot|s_t[Z_i^p], a_t[Z_i^p]))\} \\
	&\leq 2\max_{y\in \cL_{s_t,a_t}} |w_{k(t)}(y)| \sum_{i=1}^m K_{i,s_t[Z_i^p], a_t[Z_i^p]} \, ,
	}
		where for $(s,a)\in \cS\times \cA$, we define $\cL_{s,a} = \otimes_{i=1}^m \cK_{i,s[Z_i^p], a[Z_i^p]}$. 
	Since $k(t)$ is an episode where $M\in \cM_{t_k,\delta}$, we further obtain that:
$
|X_t| \leq  \max_{i,s\in \cS_i} D_{i,s}\times \max_{(s,a)\in \cX} \sum_{i=1}^m K_{i,s[Z_i^p],a[Z_i^p]} \, . 
$	
	
	%Note that $|X_t| \leq \|P(\cdot|s_t,a_t) - \mathbf e_{s_{t+1}}\|_1\frac{D}{2} \leq  D$, 
	So, $X_t$ is bounded and also $\mathbb{E}[X_t|s_1, a_1, \dots, s_t, a_t] = 0$, so that $(X_t)_t$ is martingale difference sequence. Therefore, by  Lemma  \ref{lem:bounded_peeling}, we get:
	\beqan
	\mathbb P\bigg(\exists  T: \sum_{t=1}^T X_t  \geq \max_{i,\in \cS[Z_i^p]} D_{i,s} \max_{(s,a)\in \cX} \sum_{i=1}^m K_{i,s[Z_i^p],a[Z_i^p]}\sqrt{T\beta_T(\delta)/2}\bigg)\leq \delta\,.
	\eeqan
	Hence, we deduce that with probability at least $1-\delta$, the result holds. 
\ep
	

\subsection{Other Supporting Lemmas}
\label{sec:supp_lemmas}
\noindent{\it Proof of Lemma \ref{lem:N_k_sequenence_sums}.} 
Observe that for any sequence of numbers $z_1, z_2, \dots, z_n$ with $0 \leq z_k \leq Z_{k-1} := \max\{1, \sum_{i=1}^{k-1}z_i\}$, it holds
\als{
\sum_{k=1}^n 	\frac{z_k}{\sqrt{Z_{k-1}}} 	\leq 	\big(\sqrt{2} + 1\big) 	\sqrt{Z_n} \quad \hbox{and}\quad \sum_{k=1}^n \frac{z_k}{Z_{k-1}} \leq 2\log(Z_n) + 1\, .
}
We refer to \citep[Lemma~19]{jaksch2010near} and \citep[Lemma~24]{talebi2018variance} for proof of these facts. The assertion of the lemma then easily follows by these facts and using Jensen's inequality. 
\ep

%The proof easily follow by applying Lemma \ref{lem:sequence_sums}, which is stated at the end of this proof, and using Jensen's inequality. 
%\ep
%
%\begin{lemma}[{\cite[Lemma~19]{jaksch2010near}, \cite[Lemma~24]{talebi2018variance}}]\label{lem:sequence_sums}
%	For any sequence of numbers $z_1, z_2, \dots, z_n$ with $0 \leq z_k \leq Z_{k-1} := \max\{1, \sum_{i=1}^{k-1}z_i\}$, it holds
%\als{
%(i)& \qquad \sum_{k=1}^n 	\frac{z_k}{\sqrt{Z_{k-1}}} 	\leq 	\big(\sqrt{2} + 1\big) 	\sqrt{Z_n}\, . \\
%(ii)& \qquad \sum_{k=1}^n \frac{z_k}{Z_{k-1}} \leq 2\log(Z_n) + 1\, .\\
%}
%\end{lemma}

\begin{lemma}\label{lem:factored_count}
Let $Z_1,\ldots,Z_m\subseteq [n]$, and for $x\in \cX$, let $\nu_k(x)$ denote the local counts for some episode $k$. Then, for any $i$ and any positive function $\alpha:\cX[Z_i] \to \RR$, we have: 
\als{
\sum_i \sum_{x\in \cX} \nu_k(x) \alpha(x[Z_i]) \leq  \sum_i \sum_{x'\in \cX[Z_i]} \nu_k(x')\alpha(x')\, .
}
\end{lemma}

\bp
We have:
\als{
\sum_i \sum_{x\in \cX}\nu_k(x) &\alpha(x[Z_i]) = \sum_i \sum_{x\in \cX} \sum_{t=t_k}^{t_{k+1}-1}  \indic{x_{t'} = x} \alpha(x[Z_i])\\
&= \sum_i \sum_{x'\in \cX[Z_i]}\sum_{x''\in \cX[[n]\setminus Z^p_i]}  \sum_{t=t_k}^{t_{k+1}-1}  \indic{x_{t'}[[n]\setminus Z_i] = x''} \indic{x_{t'}[Z_i] = x} \alpha(x[Z_i])\\
&= \sum_i \sum_{x'\in \cX[Z_i]} \alpha(x')  \sum_{t=t_k}^{t_{k+1}-1} \indic{x_{t'}[Z_i] = x}\underbrace{\sum_{x''\in \cX[[n]\setminus Z_i]}   \indic{x_{t'}[[n]\setminus Z_i] = x''}}_{\leq 1}
\\
&\leq \sum_i \sum_{x'\in \cX[Z_i]} \nu^p_k(x')\alpha(x')\, . 
}
\ep


%We recall the following bound on $L_1$ deviations of factored transitions.  
%
%\begin{lemma}[{Factored $L_1$ Deviations \cite[Lemma~1]{osband2014near}}]
%\label{lem:factored_deviation_L1}
%Let $\cX=\cX_1\times\cdots\cX_n$ and $\cS=\cS_1\times\cdots\times \cS_m$, and consider $P,P'\in \cP^{\textrm{fac}}_{\cX,\cS}(Z_1,\ldots,Z_m)$. We have
%\als{
%\|P-P'\|_1 &\leq \sum_{i=1}^m \|P_i(x[Z_i]) - P'_i(x[Z_i])\|_1\, .
%}
%\end{lemma}

%\section{Extended Value Iteration}


%	To upper bound $F_2$, we will need the following lemma:



\noindent{\it Proof of Lemma \ref{lem:SqrtVar_pqBern}.}
	By Taylor's expansion, we have
	\als{
		y(1-y) &= x (1- x) + (1 - 2x)(y - x) -(y - x)^2 \\
		&= x(1- x) + (1 - x - y)(y - x) \\
		&\leq
		x (1-x) + |1 - x - y |\left(\sqrt{2y (1-y)\zeta} + \tfrac{1}{3}\zeta\right) \sk
		&\leq
		x (1-x) + \sqrt{2 y(1- y)\zeta} + \tfrac{1}{3}\zeta
		\, .
	}
	Using the fact that $a\le b\sqrt{a}+c$ implies $a\le b^2 + b\sqrt{c} + c$ for nonnegative numbers $a,b$, and $c$, we get
	\begin{align}
	y(1-y)
	&\leq
	x (1-x)  + \tfrac{1}{3}\zeta + \sqrt{2\zeta\left(x (1-x)  + \tfrac{1}{3}\zeta\right)} + 2\zeta \sk
	&\leq
	x (1-x)  + \sqrt{2\zeta x (1-x)} + 3.15\zeta  \sk
	%\label{eq:P_var_1}
	&= \left(\sqrt{x (1-x)}  + \sqrt{\tfrac{1}{2}\zeta}\right)^2 + 2.65\zeta\, ,
	\end{align}
	where we have used $\sqrt{a+b}\le \sqrt{a} + \sqrt{b}$ valid for all $a,b\ge 0$. Taking square-root from both sides and using the latter inequality give the desired result:
	\begin{align*}
	\sqrt{y(1 - y)} &\leq
	\sqrt{x(1- x)} + \sqrt{\tfrac{1}{2}\zeta} + \sqrt{2.65\zeta} \leq \sqrt{x(1- x)} + 2.4\sqrt{\zeta} \, .
	\end{align*}
\ep






%\subsection{Proof of Lemma \ref{lem:factored_deviation}}
\section{Regret Analysis: Cartesian Products}
\label{app:regret_proof_Cartesian}

\subsection{Proof of Lemma \ref{lem:VI_Cartesian_prod}}
We prove the lemma by induction on $i$. 
Consider $u_0(s) = 0$. For $n=1$, we have:
\als{
u_1(s) &= \max_{a\in \cA} r(s,a) = \max_{a[1],\ldots,a[k]} \sum_{i} r^{(i)}(s[i],a[i]) = \sum_i \max_{a[i]\in \cA^{(i)}} r^{(i)}(s[i],a[i]) \, .
}
Now assume that for $n>1$, $u_n(s) = \sum_{i=1}^m u^{(i)}_{n}(s[i])$. We would like to show that $u_{n+1}(s) = \sum_{i=1}^k u^{(i)}_{n+1}(s[i])$. We have
\als{
u_{n+1}(s) &= \max_{a\in \cA}\bigg\{r(s,a) + \sum_{y\in \cS} P(y|s,a) u_n(y)\bigg\} \\
&= \max_{a_1,\ldots,a_k}\bigg\{\sum_{i} r^{(i)}(s[i],a[i]) + \sum_{y_1\in \cS^{(1)}}\ldots\sum_{y_k\in \cS^{(k)}} \prod_{i=1}^k P^{(i)}(y_i|s[i],a[i]) \sum_{j=1}^k u^{(j)}_{n}(y_j) \bigg\} \, .
}
We have
\als{
\sum_{y_1\in \cS^{(1)}}\ldots\sum_{y_m\in \cS^{(k)}} &\prod_{i=1}^k P^{(i)}(y_i|s[i],a[i]) \sum_{j=1}^k u^{(j)}_{n}(y_j) \\
 &= \sum_{j=1}^k \sum_{y_j\in \cS^{(j)}} P^{(j)}(y_j|s[j],a[j])u^{(j)}_{n}(y_j) \sum_{y \in \otimes_{i\neq j} \cS^{(i)}} \prod_{i\neq j} P^{(i)}(y_i|s[i],a[i]) \\
&= \sum_{j=1}^k \sum_{y_j\in \cS^{(j)}} P^{(j)}(y_j|s[j],a[j])u^{(j)}_{n}(y_j) \,.
}
Hence, 
\als{
u_{n+1}(s) &= \max_{a[1],\ldots,a[k]}\bigg\{\sum_{i} r^{(i)}(s[i],a[i]) + \sum_{i=1}^k \sum_{y_i\in \cS^{(i)}} P^{(i)}(y_i|s[i],a[i])u^{(i)}_{n}(y_i) \bigg\} \\
&= \sum_{i=1}^k \max_{a[i]\in \cA^{(i)}}\bigg\{r^{(i)}(s[i],a[i]) + \sum_{y_i\in \cS^{(i)}} P^{(i)}(y_i|s[i],a[i])u^{(i)}_{n}(y_i) \bigg\}\\
&= \sum_{i=1}^k u_{n+1}^{(i)}(s[i]) \, ,
}
thus concluding the lemma. 
\ep

\subsection{Proof of Theorem \ref{thm:regret_Alg1_Cartesian}}

Without loss of generality, we assume $\cG_r = \cG_p$ (and in particular, $\ell = m$), and further assume that $(Z_{i}^r)_{i\in [\ell]}$ (and so, $(Z_{i}^p)_{i\in [m]}$) forms a partition of $[n]$ -- Hence, with no loss of generality, the FMDP is assumed to be the product of $m$ base MDPs. The proof can be straightforwardly extended to the case where $\cG_r \neq \cG_p$, at the expense of more complicated and tedious notations. 

As $\cG_r = \cG_p$, in what follows we omit the dependence of scope sets or various quantities on $r$ and $p$. 
We first make the following observation, which follows by straightforward calculations: $g^\star = \sum_{i=1}^k g_i^\star$, where $g^\star_i$ denotes the optimal gain of $M^{(i)}$. %Further, the bias satisfies 
%\als{
%b^\star(s) = \EE[\sum_{t=1}^\infty (r_t - g^\star) | s_1 = s] = \sum_i \EE[\sum_{t=1}^\infty (r_{t}[i] - g^\star_i)| s_1[i] = s[i]] = \sum_{i} b^\star_i(s[i])\, ,
%}
%where for each $i\in[m]$ we define $b_i(s) = \EE[\sum_{t=1}^\infty (r_{t}[i] - g^\star_i)|s_1[i] = s]\, , \forall s\in \cS_i$.  
We have 
\als{
\kR(T) &= Tg^\star - \sum_{t=1}^T\frac{1}{m}\sum_{i=1}^m r_{t}[i] = \frac{1}{m}\sum_{i=1}^m \big(Tg^\star_i - \sum_{t=1}^T r_{t}[i]\big) \, .
}
Following similar steps as in the proof of Theorem \ref{thm:regret_Alg1}, we obtain that with probability at least $1-\delta$, 
\als{
\kR(T) \leq \sum_{k=1}^{K(T)} \Delta_k + \sqrt{T\beta_T(\delta)/2}\, ,
}
where $\Delta_k$ is defined similarly to the  proof of Theorem \ref{thm:regret_Alg1}. Now consider a good episode $k$. The corresponding optimistic policy  $\pi^+_{k}$ and $\widetilde M_{k}$ satisfy (as in the  proof of Theorem \ref{thm:regret_Alg1}): $g_k := g_{\pi^+_{k}}^{\widetilde M_{k}} \geq g^\star - \frac{1}{\sqrt{t_k}}$. In particular,  by construction $\widetilde M_k\in \mathbb M_{\cG(M)}$, and thus, $g_k = \sum_{i=1}^m g_{i,k}$, where $g_{i,k}$ denotes the average-reward of base MDP $i$ in $\widetilde M_k$. 
We therefore have:
\begin{align*}
\Delta_k  &\leq \sum_{x\in \cX} n_k(x) \frac{1}{m}\sum_{i=1}^m \big(g_{i,k} - \mu_i(x[Z_i])\big) + \sum_{x\in \cX} \frac{n_k(x)}{\sqrt{t_k}} 
\, .
\end{align*}
Leveraging the arguments in the proof of  Theorem \ref{thm:regret_Alg1}, and applying Lemma \ref{lem:VI_Cartesian_prod},\footnote{We stress that Lemma \ref{lem:VI_Cartesian_prod} applies to \EVI\ as well, as the inner maximization of \EVI\ is guaranteed to return a factored transition function.} we observe that the value function $u_k^{(l)}$ computed by \EVI\ at iteration $l$ satisfies:
\als{
u_k^{(l+1)}(s) &= \frac{1}{m}\sum_{i=1}^m \widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i]) + \sum_{s'} \widetilde P_k(s'|s,\pi^+_{k}(s)) u_k^{(l)}(s')\\
&=\frac{1}{m} \sum_{i=1}^m \Big(\widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i]) + \sum_{y_i\in \cS_i} \widetilde P_{i,k}(y_i|(s,\pi^+_{k}(s))[Z_i]) u_{i,k}^{(l)}(y_i) \Big)
\, .
} 
Now the stopping criterion of \EVI\ implies:
\begin{equation*}
\Big| \sum_{i=1}^m \Big( g_{i,k} - \widetilde\mu_{i,k}((s,\pi^+_{k}(s))[Z_i]) - \sum_{y_i\in \cS_i} \widetilde P_{i,k}(y_i|(s,\pi^+_{k}(s))[Z_i])u_{i,k}^{(l)}(y_i) + u_{i,k}^{(l)}(s[i])\Big)\Big|
\leq \frac{m}{\sqrt{t_k}}\, , \qquad \forall s\in \cS\, ,
\end{equation*}
which, after defining the corresponding matrices as done in the proof of Theorem \ref{thm:regret_Alg1}, gives
\begin{equation*}
\Big|\sum_{i=1}^m \Big({\bf g}_{i,k} - \widetilde{\boldsymbol{\mu}}_{i,k} - (\widetilde{\mathbf{P}}_{i,k} - \mathbf{I}) u_{i,k}^{(l)}\Big) \Big|
\leq \frac{1}{\sqrt{t_k}}\mathbf 1\,.
\end{equation*}
This gives
\begin{align}
\Delta_k&\leq  \frac{1}{m}\sum_{x} n_k(x)  \sum_{i=1}^m \Big(g_{i,k} -  \widetilde\mu_{i,k}(x[Z_i]) \Big) + \frac{1}{m}\sum_{x} n_k(x) \sum_{i=1}^m\Big( \widetilde\mu_{i,k}(x[Z_i]) - \mu_{i}(x[Z_i]) \Big) +  2\sum_{x} \frac{n_k(x)}{\sqrt{t_k}} \nonumber\\
&\leq  \frac{1}{m}\sum_{x} n_k(x)  \sum_{i=1}^m \Big(g_{i,k} -  \widetilde\mu_{i,k}(x[Z_i]) \Big) + \frac{1}{m}\sum_{x} n_k(x) \sum_{i=1}^m\Big( \widetilde\mu_{i,k}(x[Z_i]) - \mu_{i}(x[Z_i]) \Big) \sk
& + 2\sum_{x}  \sum_{i=1}^m \frac{n_k(x)}{\sqrt{N_{i,k}(x[Z_i])}}
\nonumber\\
&\leq    \frac{1}{m}\sum_{i=1}^m \sum_{x\in \cX[Z_i]} \nu_{i,k}(x) \Big(g_{i,k} -  \widetilde\mu_{i,k}(x) \Big) + \frac{1}{m}\sum_x \sum_{i=1}^m n_k(x)\frac{2\beta'_{T,i}}{\sqrt{N_{i,k}(x[Z_i])}}  +  2\sum_{i=1}^m \sum_{x\in \cX[Z_i]} \frac{\nu_{i,k}(x)}{\sqrt{N_{i,k}(x)}} \nonumber\\
&\leq \frac{1}{m}\sum_{i=1}^m \nu_{i,k} (\widetilde{\mathbf{P}}_{i,k} - \mathbf{I} ) u_{i,k}^{(l)} + \frac{1}{m}\sum_{i=1}^m \beta'_{T,i}\sum_{x\in \cX[Z_i]} \frac{\nu_{i,k}(x)}{\sqrt{N_{i,k}(x)}} +  2\sum_{i=1}^m \sum_{x\in \cX[Z_i]} \frac{\nu_{i,k}(x)}{\sqrt{N_{i,k}(x)}}  \, .\nonumber
\end{align}
Here, we used the fact that $t_k\ge \max_{i\in [m]} N_{i,k}(x[Z_i])$, and applied Lemma \ref{lem:factored_count}. 

Now defining for each $i$, $w_{i,k}(s) := u_{i,k}^{(l)}(s) - \tfrac{1}{2}(\min_s u_{i,k}^{(l)}(s) + \max_s u_{i,k}^{(l)}(s))$ for all $s\in \cS_i$, we arrive at
$\Delta_k\leq \frac{1}{m}\sum_{i=1}^m \widetilde \Delta_{i,k}$ with 
\als{
\widetilde \Delta_{i,k} := \nu_{i,k} (\widetilde{\mathbf{P}}_{i,k} - \mathbf{I} ) u_{i,k}^{(l)} + \beta'_{T,i} \sum_{x\in \cX[Z_i]} \frac{\nu_{i,k}(x)}{\sqrt{N_{i,k}(x)}} +  2 \sum_{x\in \cX[Z_i]} \frac{\nu_{i,k}(x)}{\sqrt{N_{i,k}(x)}} \, . 
}
In other words, the regret is upper bounded by a quantity, which only depends on the properties of MDP $M^{(i)}$. Following exact same arguments as in the rest of proof of Theorem \ref{thm:regret_Alg1} (or similarly, those in the proof of Thoerem 1 in \citep{bourel2020tightening}) gives the desired result. 
\ep





==> sections/simulation_arXiv.tex <==

\section{Numerical Experiments}\label{sec:xps}

In this section we present results from numerical experiments with \AlgB. We perform experiments with the algorithm in two domains: a factored version of RiverSwim \cite{strehl2008analysis,filippi2010optimism}, and the Coffee domain \cite{boutilier1994fmdps} in which a robot has to bring coffee to its user. For RiverSwim, we construct an FMDP by taking the Cartesian product of two RiverSwim instances with 6 states each, and introduce additional reward for a single joint state to couple the two instances through the reward factors. This corresponds to $S=36$ and $A=4$ (and so, $|\cX|=144$). For Coffee, since the original domain is episodic, we introduce a reset action that returns the robot to an initial state from any terminal state, at the expense of slightly increasing the scope of the transition factors. The size of this domain is $S=64$, $A=4$, and $|\cX|=256$. 
Recall that $\cX = \cS_1\otimes\cdots\otimes\cS_m\otimes\cA_1\otimes\cdots\otimes\cA_{n-m}$, i.e. each factor scope $\cX[Z_i^p]$ (resp.~$\cX[Z_i^r]$) is the Cartesian product of a subset of state and action factors. In other words, the learner knows which subset of factors is relevant for transition factor $P_i$ (resp.~reward factor $R_i$), but does not have access to a compact representation, e.g.~in the form of a decision tree. Having access to such a compact representation would improve the performance of the algorithm, but makes a stronger assumption on the available prior knowledge .

We compare \AlgB{} to the following algorithms: UCRL2B, a variant of UCRL2 relying on the same confidence sets for reward and transition function but ignoring the factored structure; 
UCRL-Factored \citep{osband2014near}, the previous state-of-the-art algorithm for FMDPs; UCRL-Factored-L, a variant of UCRL-Factored with improved confidence intervals derived from tight time-uniform $L_1$-type confidence sets. Though the latter algorithm was never published, we include it to illustrate that the gain of \AlgB{} is not only due to tighter confidence intervals, but comes also from maintaining element-wise Bernstein-type sets; we refer to the supplementary material for further details. 
In particular, comparison against UCRL2B indicates the gain achieved by taking into account the factored structure, whereas that against UCRL-Factored and UCRL-Factored-L
reveals the gain of (element-wise) Bernstein-type confidence sets over their $L_1$-type counterparts. 
We remark that we do not compare to PSRL \citep{osband2014near,xu2020near} since it has only shown to guarantee a Bayesian regret bound, and to the best of our knowledge, its frequentist regret analysis is still open.
As far as we know, ours is the first full-scale empirical evaluation of regret minimization algorithms for FMDPs; \citep{xu2020near} perform limited experiments with PSRL and do not compare to UCRL2. 
%Due to numerical instability, we only use Bernstein-derived confidence intervals in \AlgB{} and UCRL3-with-EVI. 

% the state-of-the-art regret minimization algorithm for non-factored MDPs; 

\begin{figure}[tpb]
	\centering
	\begin{minipage}{0.46\textwidth}
		\centering
	    \includegraphics[scale=1.46]{images/riverswim_regret_c.pdf}

	   % \vspace{-0.3cm}

	    \caption{Regret over time in RiverSwim.}
		\label{fig:riverswim-regret}
	\end{minipage}\hfill
	\begin{minipage}{0.53\textwidth}
		\centering
		\includegraphics[scale=1.22]{images/coffee_regret_c.pdf}

	%	\vspace{-0.3cm}

		\caption{Regret over time in Coffee.}
		\label{fig:coffee-regret}
	\end{minipage}

	%\vspace{-0.5cm}
\end{figure}

In our experiments, we set $\delta=0.01$ and report for each domain the average results over 48 independent experiments. 
Figure~\ref{fig:riverswim-regret} shows the regret of various algorithms as a function of rounds in RiverSwim. As the figure reveals, the regret under \AlgB\ significantly improves over that of other algorithms. In particular, \AlgB{} enjoys a very short \emph{burn-in} phase, after which the regret grows sublinearly with time. We also note that in this domain, Factored-UCRL-L dominates UCRL2B, implying that taking the structure into account is important. In Figure~\ref{fig:coffee-regret}, we report the regret under various algorithms over time in the Coffee domain. As the figure presents, \AlgB\ admits a much shorter burn-in phase than the others: While around time $t=4\times 10^5$ \AlgB\ already enters the sublinear phase, the rest still are in the linear phase by $t=10^6$. By continuing this task for much larger horizon, one would see that a similar trend as in Figure \ref{fig:riverswim-regret}. 
We provide additional numerical experiments in the supplementary material. UCRL-Factored-L did not outperform UCRL-Factored in the Coffee domain which is why we omit the algorithm from the figure.
Additional experiments are reported in Appendix \ref{app:additional_sim}).

